Isolating Bounded and Unbounded Real Roots of a Mixed Trigonometric-Polynomial

Mixed trigonometric-polynomials (MTPs) are functions of the form $f(x,\sin{x}, \cos{x})$ with $f\in\mathbb{Q}[x_1,x_2,x_3]$. In this paper, an algorithm ``isolating" all the real roots of an MTP is provided and implemented. It automatically divides the real roots into two parts: one consists of finitely many ``bounded" roots in an interval $[\mu_-,\mu_+]$ while the other consists of probably countably many ``periodic" roots in $\mathbb{R}\backslash[\mu_-,\mu_+]$. For bounded roots, the algorithm returns isolating intervals and corresponding multiplicities while for periodic roots, it returns finitely many mutually disjoint small intervals $I_i\subset[-\pi,\pi]$, integers $c_i>0$ and multisets of root multiplicity $\{m_{j,i}\}_{j=1}^{c_i}$ such that any periodic root $t>\mu_+$ is in the set $(\sqcup_i\cup_{k\in\mathbb{N}}(I_i+2k\pi))$ and any interval $I_i+2k\pi\subset(\mu_+,\infty)$ contains exactly $c_i$ periodic roots with multiplicities $m_{1,i},...,m_{c_i,i}$, respectively. The effectiveness and efficiency of the algorithm are shown by experiments. %In particular, our results indicate that the ``distributions" of the roots of an MTP in the ``periods" $(-\pi,\pi]+2k\pi$ sufficiently far from $0$ share a same pattern. Besides, the method used to isolate the roots in $[\mu_-,\mu_+]$ is applicable to any other bounded interval as well. The algorithm takes advantages of the weak Fourier sequence technique and deals with the intervals period-by-period without scaling the coordinate so to keep the length of the sequence short. The new approaches can easily be modified to decide whether there is any root, or whether there are infinitely many roots in unbounded intervals of the form $(-\infty,a)$ or $(a,\infty)$ with $a\in\mathbb{Q}$.

==> Isolating all the Real Roots of a Trigonometric-Polynomial/alg/alg7.tex <==
\begin{algorithm}[!t]\label{alg:CompleteAlgorithm}
\tiny
\DontPrintSemicolon
\LinesNumbered
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{ 
  $f(x,\tau,\upsilon)\in \Q[x,\tau,\upsilon]$;\\
  a positive rational number $\varepsilon$ that specifies the maximal length of isolating intervals.
}
\Output{\\
a finite set of some $2$-tuples $\{([[\alpha_i,\beta_i]],m_i)\}_i$, where $\alpha_i,\beta_i\in (2\arctan(\Q)+\frac{\Z}{2}\pi)\cup\Q$, such that for every $i$, there is $1$ real root  of $f(x,\sin x,\cos x)$ in $[[\alpha_i,\beta_i]]$ and the root is of multiplicity $m_i$;\\
a finite set of some $3$-tuples $\{([[\alpha_i,\beta_i]],(c_i,m_i),k_i)\}_i $, where $\alpha_i,\beta_i\in 2\arctan(\Q)+\frac{\Z}{2}\pi$, such that for every $i$: if $k_i\ge 0$,  there are exactly $c_i$ roots of $f(x,\sin x,\cos x)$ in $[[\alpha_i,\beta_i]]+2k\pi\ (k\ge k_i)$ and each root is of multiplicity $m_i$;
if $k_i< 0$, there are exactly $c_i$ roots of $f(x,\sin x,\cos x)$ in $[[\alpha_i,\beta_i]]+2k\pi\ (k\le k_i)$ and each root is of multiplicity $m_i$.
}
\caption{\bf Main Algorithm}\label{alg:complete-algorithm}
\BlankLine
 $ans_1\leftarrow \emptyset$; $ans_{2}\leftarrow \emptyset$; $g\leftarrow f(2 x,\frac{2 y}{1+y^2},\frac{1-y^2}{1+y^2})\cdot (y^2+1)^{\tdeg(f,[\tau,\upsilon])}$\;
\If{\label{algline:whetherg0}$g$ is the zero polynomial}{
    \textbf{ERROR} ``$f(x,\sin x,\cos x)$ is identically zero" \;\label{algline:error}
}
 $gcot\leftarrow f(2 x,\frac{2 y}{1+y^2};  \frac{y^2 - 1}{1+y^2})\cdot (1 + y^2)^{\tdeg(f, [\tau,\upsilon])}$\;
Let $m_1$ be the maximal positive integer such that $y^{m_1}|gcot$\;\label{algline:m1}
\If{$m_1\neq 0$}{
$ans_2$.add($([\pi,\pi],(1,m_1),0)$); $ans_2$.add($([\pi,\pi],(1,m_1),-1)$)\;
}
\If{$f(0,\sin0,\cos0)=0$}{
    $m_2\leftarrow$ the multiplicity of $f(x,\sin{x},\cos x)$ at $0$; $ans_1$.add($([0,0],m_2)$)\;
}
Let $m_3$ be the maximal positive integer such that $y^{m_3}|g$\;
\If{$m_3\neq 0$}{
    $ans_2$.add($([0,0],(1,m_3),1)$); $ans_2$.add($([0,0],(1,m_3),-1)$); $g\leftarrow g/y^{m_3}$\;
}\label{algline:m3}
$(a_1,b_1),\ldots, (a_s,b_s)\leftarrow$ the isolating  intervals of $\lc(g,x)$ such that $\arctan b_i -\arctan a_i <\varepsilon/2~(1\le i\le s)$\;\label{algline:isolate}
% Isolate all real roots of $\lc(g,x)$ , and denote the isolating  intervals by $(a_1,b_1),\ldots, (a_s,b_s)$ such that $\arctan b_i -\arctan a_i <\varepsilon/2$ for all $i~(1\le i\le s)$.\; 
$a_0\leftarrow-\infty$; Let $b_0\in\Q$ such that $\arctan b_0- (-\frac{\pi}{2})< \frac{\varepsilon}{2}$ and $b_0< a_1$.\; 
$b_{s+1}\leftarrow+\infty$; Let $a_{s+1}\in\Q$ such that $ \frac{\pi}{2}-\arctan a_{s+1}< \frac{\varepsilon}{2}$ and $a_{s+1}> b_s$.\; 
$I\leftarrow [(a_0,b_0),\ldots,(a_{s+1},b_{s+1})]$\;\label{algline:PPIS}
Factorize $g$ as ${c_0}\prod_{i=1}^{n} g_i^{p_i}$\;\label{algline:factorize}
$ans_{21}\leftarrow \emptyset;~ans_{22}\leftarrow \emptyset$; $k_-\leftarrow 0$; $k_+\leftarrow 0$\;
\For{$i$ from 1 to $n$}{
    \eIf{$\deg(g_i,y)\geq 1$}{\label{algline:deggy>0part}
        $k^*_1, \{((\alpha_{j},\beta_{j}),c_{j}) \}_j$ $\leftarrow$ Call Algorithm \ref{alg:AlgDerBound} with $g_i(x,y)$ and $I$\;
        $k_+\leftarrow\max\{k^*_1, k_+\}$; $ans_{21}$.add($\{((2\alpha_{j},2\beta_{j}),(c_{j},p_i)) \}_j$)\;\label{algline:renewk+}
        $k^*_2, \{((\alpha_{j},\beta_{j}),c_{j}) \}_j$ $\leftarrow$ Call Algorithm \ref{alg:AlgDerBound} with $g_i(-x,-y)$ and $I$\;
        $k_-\leftarrow\min\{-k^*_2,k_-\}$; $ans_{22}$.add($\{((-2\beta_{j},-2\alpha_{j}),(c_{j},p_i)) \}_j$)\;\label{algline:renewk-}
    }
    {
            %Let $\tilde{g}\in\Q[x]$ be the product of those $g_i$ \emph{s.t.} $\deg(g_i, y)=0$\;
        $\{[[\alpha_{j},\beta_{j}]]\}_j\leftarrow$   the isolating  intervals of nonzero roots of ${g_i}$ such that they do not intersect $[0,0]$ and $\beta_{j} - \alpha_{j}<\varepsilon/2$.\;\label{algline:isolateAlge}
        %Remove $[0,0]$ in  $\{[[\alpha_{j},\beta_{j}]]\}_j$;
        $ans_1$.add($\{([[2\alpha_{j},2\beta_{j}]],p_i)\}_j$)\;\label{algline:remove00}
        % $S\leftarrow$ All real roots of $g_i(x)$\;
        % $k_-\leftarrow \min \{k_-,\min_{x\in S} \lfloor \frac{x}{\pi}+\frac{1}{2}\rfloor\}$; $k_+\leftarrow \max \{k_+,\max_{x\in S} \lceil \frac{x}{\pi}-\frac{1}{2}\rceil\}$\;
        
    }
}
Refine the intervals obtained in the ``\textbf{else}" part of the above loop so that they do not intersect.\;
\For{each $((\alpha^*,\beta^*),(c^*,p^*))$ in $ans_{21}$\label{algline:unifyk+}}{
    $ans_2$.add($((\alpha^*,\beta^*),(c^*,p^*),k_++1)$)\;
}
\For{each $((\alpha^*,\beta^*),(c^*,p^*))$ in $ans_{22}$}{
    $ans_2$.add($((\alpha^*,\beta^*),(c^*,p^*),k_--1)$)\;
}\label{algline:unifyk-}


\For{$k$ from $k_-$ to $k_+$}{\label{algline:k-tok+}
    \For{$i$ from 1 to $n$}{
        \If{$\deg(g_i,y)\geq 1$}{
            $\{[[\alpha_{j},\beta_{j}]]\}_j\leftarrow$ Call Algorithm \ref{alg:BoundRSI} with $g_i(x,y)$ and $k$\;
             Remove $[0, 0]$ in  $\{[[\alpha_{j},\beta_{j}]]\}_j$; 
             % and refine every $[[\alpha_{j},\beta_{j}]]$ such that $\beta_{j} - \alpha_{j}<\varepsilon/2$.\;
          $ans_1$.add($\{([[2\alpha_{j},2\beta_{j}]],p_i)\}_j$)\;\label{algline:Remove0}
        }
    }
    Refine the intervals  $[[\alpha_{j},\beta_{j}]]$  obtained in the above loop so that any two of them do not intersect and $\beta_{j} - \alpha_{j}<\varepsilon/2$.\;\label{algline:refineboundedroots}
}


\Return  $ans_1$, $ans_2$\;
\end{algorithm}

==> Isolating all the Real Roots of a Trigonometric-Polynomial/chap/Boundedsolve.tex <==
\section{Isolating Bounded Real Roots}\label{sec:IBR}
In this section, we discuss case \ref{item:MainThreeCase1} in Section \ref{sec:Preprocessing}, i.e., given $k_+,k_-\in\Z$, isolating the real roots of
\begin{align}\label{eq:boudedeq}
    g(x,\tan x)=0,~~~~x\in(k\pi-\frac{\pi}{2},k\pi+\frac{\pi}{2})
    %~{\rm where}~k_-\le k\le k_+.
\end{align}
where $g\in\Q[x,y]\setminus\{0\}$, $k\in\Z$ and $k_-\le k\le k_+$.

We solve \eqref{eq:boudedeq} in four intervals $(k\pi-\frac{\pi}{2},k\pi-\frac{\pi}{4}),(k\pi-\frac{\pi}{4},k\pi),(k\pi,k\pi+\frac{\pi}{4})$ and $(k\pi+\frac{\pi}{4},k\pi+\frac{\pi}{2})$.
In each interval, the problem is equivalent to isolating the roots of some $G(r\pi+\arctan{y},y)$ on $(0,1)$ where $G\in\Q[x,y]$ and $r\in\Q$, and thus we can use the frame of \cite[Algorithm 47]{strzebonski2012real} to deal with it.
In Section \ref{subsec:WeakFourierSeq}, we use Algorithm \ref{alg:WeakFourierSeq} to compute a weak Fourier sequence for $G(r\pi+\arctan{y},y)$.
In fact, Algorithm \ref{alg:WeakFourierSeq} is a simplified version of \cite[Algorithm 40]{strzebonski2012real} for our specific needs.
In Section \ref{subsec:IsoRoot}, Algorithm \ref{alg:BoundRSI} is proposed to isolate the real roots of Eq. \eqref{eq:boudedeq}.

\subsection{Weak Fourier sequences}\label{subsec:WeakFourierSeq}
% \begin{definition}
% For $f(x,y)\in\Q[x,y]$, we call $f(x,\arctan(x))$ an arctangent function polynomial, denoted as arctangent-polynomial simply.
% \end{definition}

Let us first review the definition of weak Fourier sequences and an important result about it.

\begin{definition}\cite[Def. 10]{strzebonski2012real}\label{def:WeakFourierSeq}
Let $I\subseteq\R$ be an open interval, and $G_1,\ldots,G_k:I\rightarrow\R$ be a sequence of differentiable functions defined on $I$.
The sequence $G_1,\ldots,G_k$ is a \emph{weak Fourier sequence on $I$}, if for all $y\in I$,
\begin{enumerate}
    %\item $G_1(y)=G(y)$,
    \item for all $i\;(1\le i\le k-1)$, $\sign(G_{i+1}(y))=\sign(G_i'(y))$, and
    \item $G_k(y)\ne0$.
\end{enumerate}
We say $G_1,\ldots,G_k$ is a \emph{weak Fourier sequence for $G$ on $I$}, if $G_1,\ldots,G_k$ is a weak Fourier sequence on $I$ and $G_1(y)=G(y)$ for all $y\in I$.
\end{definition}

\begin{notation}
Let $a,b\in\R$ and $G_1,\ldots,G_k$ be a weak Fourier sequence on the open interval $(a,b)$.
Then, for any $i,j\;(1\le i\le j\le k)$,
\begin{enumerate}
    \item $\sign(G_{i}(x^{+})):=\sign(G_i(c))$, where $x\in[a,b)$, $c< b$ and $\forall y\in(x,c]\;G_i(y)\ne0$,
    \item $\sign(G_{i}(x^{-})):=\sign(G_i(d))$, where $x\in(a,b]$, $a< d$ and $\forall y\in[d,x)\;G_i(y)\ne0$,
    \item $\sgc_{i,j}(x)$, for $x\in(a,b)$, is the number of sign changes in the sequence $G_{i}(x),\ldots,G_{j}(x)$ with terms equal to zero removed,    
    \item $\sgc_{i,j}(x^{+})$, for $x\in[a,b)$, is the number of sign changes in the sequence $G_{i}(x^{+}),\ldots,G_{j}(x^{+})$,
    \item $\sgc_{i,j}(x^{-})$, for $x\in(a,b]$, is the number of sign changes in the sequence $G_{i}(x^{-}),\ldots,G_{j}(x^{-})$.
\end{enumerate}
\end{notation}

\begin{theorem}\cite[Thm. 13]{strzebonski2012real}\label{thm:WeakFourierSeq}
Let $I\subseteq\R$ be an open interval and let 
$G_1,\ldots,G_{k}:I\rightarrow\R$ be a weak Fourier sequence.
Then for any $x\in I$, $\sgc_{1,k}(x^{+})=\sgc_{1,k}(x)$ and $\sgc_{1,k}(x^{-})=\sgc_{1,k}(x)+r+2s$, where $r,s\in\N$ and $G_1(x)=\cdots=G_r(x)=0,G_{r+1}(x)\ne0$.
Moreover, $s=0$ unless there is a $t>r+1$ such that $G_{t}(x)=0$.\qed
\end{theorem}

Let $a,b$ be two real numbers such that $(a,b)\subseteq I$.
Remark that by the proof of \cite[Prop. 15]{strzebonski2012real}, if $\sgc_{1,k}(a^{+})=\sgc_{1,k}(b^{-})$, then $G_1$ has no real root in $(a,b)$, and if $\sgc_{1,k}(a^{+})=\sgc_{1,k}(b^{-})+1$, then $G_1$ has exactly one simple root in $(a,b)$.

To illustrate Algorithm \ref{alg:WeakFourierSeq}, we introduce the definition of the \emph{arctan-derivative}.
% Then, we define the arctan-derivative in order to compute the weak Fourier sequence we need. 

\begin{definition}\label{def:pseudo}
For any $G\in\Q(y)[x]$, let
\[
{\trueder G}:=\frac{\partial G}{\partial x}\cdot\frac{1}{1+y^2}+\frac{\partial G}{\partial y}\in\Q(y)[x].
\]
The \emph{arctan-derivative} of $G$ is defined as $G^{\pder}:={\trueder G}\cdot h(y)$, where $h(y)\in\Q[y]$ is the denominator of $\lc({\trueder G},x)\in\Q(y)$.
In particular, if $\lc({\trueder G},x)$ is a polynomial, then $h(y)=1$.
We call $h(y)$ the \emph{common-term} of $G^{\pder}$.
% where ${\trueder f}\in\Q(x)[y]$.
% If $\lc({\trueder G},x)$ is a polynomial,  and the \emph{common-term} of the arctan-derivative is $1$.
% Otherwise, let $h(y)\in\Q[y]$ be the common denominator of $\lc({\trueder G},x)$.
% The arctan-derivative of $G$ is is defined as $G^{\pder}:={\trueder G}h(y)$, and the common-term of the arctan-derivative is $h(y)$. 
%We denote by $G^{\pder}$ the arctan-derivative of $G$ and $G^{\pder}\in\Q(y)[x]$. 
\end{definition}

\begin{remark}\label{remark:def:pseudo}
For any $G\in\Q(y)[x]$, $G^{\pder}\in\Q(y)[x]$ and $\lc(G^{\pder},x)$ is a polynomial in $\Q[y]$.
\end{remark}

Given $G(x,y)\in\Q[x,y]\setminus\{0\}$ and $r\in\Q$,
the process of Algorithm \ref{alg:WeakFourierSeq} is as follows:
% we use Algorithm \ref{alg:WeakFourierSeq} to compute a weak Fourier sequence for $G(r\pi+\arctan y,y)$ on $\R$. 
Let $G_1$ be $G(x,y)$.
If $G_1$ is not a nonzero rational number, then compute the arctan-derivative $G_{1}^{\pder}$ of $G_1$, and set $G_2=G_{1}^{\pder}$.
If $G_2$ is not a nonzero rational number, then set $G_3=G_{2}^{\pder}$.
Repeat the process until some $G_k\;(k\ge1)$ is a nonzero rational number.
Then $G_1(r\pi+\arctan y,y),\allowbreak\ldots,G_k(r\pi+\arctan y,y)$ is a weak Fourier sequence for $G(r\pi+\arctan y,y)$ on $\R$.

\begin{algorithm}[!ht]
\scriptsize
\DontPrintSemicolon
\LinesNumbered
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{ $G(x,y)$, a polynomial in $\Q[x,y]\setminus\{0\}$; $r$, a rational number
}
\Output{$G_1(r\pi+\arctan{y},y),\ldots,G_k(r\pi+\arctan{y},y)$, a weak Fourier sequence for $G(r\pi+\arctan{y},y)$ on $\R$, where $G_i\in\Q(y)[x]$
}
\caption{{\bf WeakFourierSeq}}\label{alg:WeakFourierSeq}
\BlankLine
$G_1\leftarrow G(x,y)$\;
$i\leftarrow1$\;
\While{$G_i(x,y)$ is not a nonzero rational number}
{ $G_{i+1}(x,y)\leftarrow G_{i}^{\pder}(x,y)$\;
  $i\leftarrow i+1$
}
\Return{$G_1(r\pi+\arctan{y},y),\ldots,G_k(r\pi+\arctan{y},y)$}
\end{algorithm}

Note that we can easily obtain a weak Fourier sequence from a \emph{semi-Fourier sequence} (defined in \cite[Def. 14]{strzebonski2012real}) by \cite[Prop. 15]{strzebonski2012real}.
So, Algorithm \ref{alg:WeakFourierSeq} and \cite[Algorithm 40]{strzebonski2012real} are essentially the same when computing a weak Fourier sequence for $G(r\pi+\arctan{y},y)$, and thus the termination and correctness of Algorithm \ref{alg:WeakFourierSeq} are clear.
However, in order to explain some properties that will be used later, we prepare some lemmas and re-prove the termination and correctness of Algorithm \ref{alg:WeakFourierSeq}.

\begin{lemma}\label{lemma:DerEquiv0}
If $G\in\Q(y)[x]\setminus\Q$ such that $G(x,y)$ is well-defined on the whole plane $\R^2$,
then $G^{\pder}\in\Q(y)[x]\setminus\{0\}$.
% and $\lc(G^{\pder},x)$ is a polynomial.
% and $G^{\pder}\equiv0$, then $G\in\Q$.
% If $f(x,y)\in\Q(x)[y]\setminus\Q$, then ${\trueder f}(x,y)\in\Q(x)[y]\setminus\{0\}$.
\end{lemma}
\begin{proof}
Assume that $G^{\pder}$ is the zero polynomial in $\Q(y)[x]$.
By Definition \ref{def:pseudo}, ${\trueder G}$ is also the zero polynomial.
Then, ${\trueder G}(\arctan{y},y)\equiv0$.
Note that ${\trueder G}(\arctan{y},y)=\frac{\der G(\arctan{y},y)}{\der y}$.
So, $G(\arctan{y},y)\in\Q$ for any $y\in\R$. Since the arctangent function is not algebraic, $G\in\Q$, a contradiction.
% which contradicts the fact that $f(x,y)\in\Q(x)[y]\setminus\Q$.
% Therefore, ${\trueder f}(x,y)\not\equiv0$.
%\qed
\end{proof}

\begin{lemma}\label{lemma:pseudoproperty}
If $G\in\Q(y)[x]\setminus\Q$ and $\lc(G,x)$ is a polynomial, then
\begin{align}\label{eq:lemma:pseudoproperty}
    (\deg(G,x),\deg(\lc(G,x)))\succlex(\deg(G^{\pder},x),\deg(\lc(G^{\pder},x))),
\end{align}
where $\succlex$ denotes the lexicographic ordering.
\end{lemma}
\begin{proof}
Recall Remark \ref{remark:def:pseudo}. The degrees $\deg(G^{\pder},x)$ and $\deg(\lc(G^{\pder},x))$ are well-defined.

If $\deg(G,x)=0$, we have $G\in\Q(y)\setminus\Q$, and thus $\lc(G,x)=G$.
So, $G$ is a polynomial in $\Q[y]\setminus\Q$.
It is easy to check that $G^{\pder}=\frac{\partial G}{\partial y}\in\Q[y]$. 
So, $\deg(\lc(G,x))=\deg(G)$, $\deg(G^{\pder},x)=0$ and $\deg(\lc(G^{\pder},x))=\deg(G)-1$. 
Then inequality \eqref{eq:lemma:pseudoproperty} holds.

If $\deg(G,x)\ge1$, suppose that 
\begin{align}\label{eq:G}
G=a_n(y)x^n+\sum_{j=0}^{n-1}a_j(y)x^j%+a_0(y),
\end{align}
where $n=\deg(G,x)\ge1$, $a_n(y)\in\Q[y]$ and $a_j(y)\in\Q(y)$ for $j=0,\ldots,n-1$.
Then,
\begin{align}\label{eq:truederG}
    {\trueder G}=a_n'(y)x^n+&\sum_{j=0}^{n-1}\big(a_j'(y)+\frac{(j+1)a_{j+1}(y)}{1+y^2}\big)x^{j}.
    %+&\frac{(1+y^2)a_0'(y)+a_1(y)}{1+y^2}.
\end{align}
If $a_{n}'(y)$ is the zero polynomial, we have $\deg({\trueder G},x)<\deg(G,x)$.
By Definition \ref{def:pseudo}, $\deg(G^{\pder},x)=\deg({\trueder G},x)$.
So, $\deg(G^{\pder},x)<\deg(G,x)$ and inequality \eqref{eq:lemma:pseudoproperty} is true.
If $a_{n}'(y)$ is not the zero polynomial, then $\deg({\trueder G},x)=\deg(G,x)$.
Since $\lc({\trueder G},x)=a_{n}'(y)\in\Q[y]$, $G^{\pder}={\trueder G}$. Thus $\deg(G^{\pder},x)=\deg(G,x)$.
We also note that $\deg(\lc(G,x))=\deg(a_n(y))$ and $\deg(\lc(G^{\pder},x))=\deg(a_n(y))-1$.
The proof is completed.
%\qed
\end{proof}

\begin{lemma}\label{lemma:DerForm}
If $G\in\Q(y)[x]$ has the following form
\begin{align}\label{eq:specialform}
    G=a_n(y)x^{n}+\sum_{j=0}^{n-1}\frac{a_j(y)}{(1+y^2)^{m_j}}x^{j},%+\frac{a_0(y)}{(1+y^2)^{m_0}},
\end{align}
where $n=\deg(G,x)$, $a_i(y)\in\Q[y]\;(0\le i\le n)$ and $m_j\in\N~(0\le j\le n-1)$, then the common-term of $G^{\pder}$ is $(1+y^2)^m$ for some $m\in\N$.
Furthermore, $G^{\pder}$ also has the form in Eq. \eqref{eq:specialform}.
\end{lemma}
\begin{proof}
If $\deg(G,x)=0$, then $G=a_n(y)\in\Q[y]$, and thus $G^{\star}=G'(y)$, the common-term of $G^{\star}$ is $1$.
If $\deg(G,x)\ge1$, by Eq. \eqref{eq:G} and Eq. \eqref{eq:truederG} in the proof of Lemma \ref{lemma:pseudoproperty}, there exist $b_i(y)\in\Q[y]\;(0\le i\le n)$ and $d_j\in\N~(0\le j\le n-1)$ such that
\begin{align*}
    {\trueder G}=b_n(y)x^n+\sum_{j=0}^{n-1}\frac{b_j(y)}{(1+y^2)^{d_j}}x^{j}.%+\frac{b_0(y)}{(1+y^2)^{d_0}}.
\end{align*}
If $b_n(y)$ is not the zero polynomial, the common-term of $G^{\pder}$ is $1$.
Otherwise, since $\deg(G,x)\ge1$ and $G$ is well-defined on the whole $\R^2$, by the proof of Lemma \ref{lemma:DerEquiv0}, ${\trueder G}$ is not the zero polynomial.
So, there exists an integer $0\le k\le n-1$ such that $b_k(y)$ is not the zero polynomial. Let $k_0$ be the maximal one of such $k$. Then, the common-term of $G^{\pder}$ is $(1+y^2)^{d_{k_0}}$.
Therefore, $G^{\pder}$ has the same form as in Eq. \eqref{eq:specialform}.
%\qed
\end{proof}

\begin{theorem}\label{thm:alg:WeakFourierSeqTC}
   Algorithm \ref{alg:WeakFourierSeq} terminates correctly.
\end{theorem}
\begin{proof}
(Termination) 
For any $G(x,y)\in\Q[x,y]\setminus\{0\}$,
let $G_1:=G(x,y),G_2:=G_1^{\pder}(x,y),G_3:=G_2^{\pder}(x,y),\ldots$
We only need to prove that there exists $k\;(k\ge1)$ such that $G_k(x,y)$ is a nonzero rational number.
If $G_1\in\Q\setminus\{0\}$, then we take $k=1$.
If $G_1\in\Q[x,y]\setminus\Q$, then by Lemma \ref{lemma:pseudoproperty}, we have 
$$(\deg(G_1,x),\deg(\lc(G_1,x)))\succlex(\deg(G_2,x),\deg(\lc(G_2,x))).$$
Recall Remark \ref{remark:def:pseudo}. For any $i~(i\ge2)$, $G_i\in\Q(y)[x]$ and $\lc(G_i,x)$ is a polynomial.
Therefore, assume that $G_2\notin\Q$, $G_3\notin\Q$,..., by Lemma \ref{lemma:pseudoproperty}, we have
\begin{align*}
(\deg(G_1,x),\deg(\lc(G_1,x)))&\succlex(\deg(G_2,x),\deg(\lc(G_2,x)))\\
&\succlex(\deg(G_3,x),\deg(\lc(G_3,x)))\succlex\cdots.
\end{align*}
So, there exists $m\;(m\ge2)$ such that $G_m\in\Q$.
Let $k\;(k\ge2)$ be the smallest integer such that $G_k\in\Q$.
Then, $G_{k-1}\notin\Q$.
Note that $G_{k-1}$ is well-defined on the whole $\R^2$ by Lemma \ref{lemma:DerForm}.
So, by Lemma \ref{lemma:DerEquiv0}, $G_k$ is a nonzero rational number.

(Correctness) 
For $i=1,\ldots,k-1$, let $h_i(y)$ be the common-term of $G_i^{\pder}(x,y)$.
Recall Definition \ref{def:pseudo}. 
We have $G_{i+1}(x,y)=h_i(y){\trueder G}_{i}(x,y)$.
% So, $f_{i+1}(x,y)={\trueder f}_{i}(x,y)h_i(x)$.
Note that 
$${\trueder G}_{i}(r\pi+\arctan{y},y)=G_i(r\pi+\arctan{y},y)'$$
and $G_{i+1}(x,y)\in\Q(y)[x]$.
Thus, we only need to prove that $\sign(h_i(y))>0$ on the whole $\R$ and $G_{i+1}(r\pi+\arctan{y},y)$ is defined on the whole $\R$.
If $\deg(G,x)=0$, then $G\in\Q[y]$.
So, $h_i(y)=1$ and $G_{i+1}(r\pi+\arctan{y},y)$ is defined on the whole $\R$.
If $\deg(G,x)\ge1$, 
by the termination proof, there exists $m\;(1\le m\le k-1)$ such that $\deg(G_1,x)\ge1,\ldots,\deg(G_m,x)\ge1$ but $\deg(G_{m+1},x)=0$.
Applying Lemma \ref{lemma:DerForm} to $G_i\;(i=1,\dots,m)$, we have 
$h_i(y)=(1+y^2)^{n_i}\;(n_i\in\N)$ and $G_{i+1}(r\pi+\arctan y,y)$ is defined on the whole $\R$.
Since $\deg(G_{m+1},x)=0$, $G_{m+1}\in\Q[y]$.
So, for any $m+1\le i\le k-1$, $h_i(x)=1$ and %\textcolor{blue}{$G_{i+1}(r\pi+\arctan y,y)$, with
$G_{i+1}\in\Q[y]$, which is also defined on the whole $\R$.
%\qed
\end{proof}

\begin{remark}\label{remark:PolyWeakFourierSeq}
Let $G(x,y)\in\Q[x,y]\setminus\{0\}$, $r\in\Q$ and $G_1(r\pi+\arctan{y},y),\ldots,\allowbreak G_k(r\pi+\arctan{y},y)$ be a weak Fourier sequence for $G(r\pi+\arctan{y},y)$ on $\R$ computed by Algorithm \ref{alg:WeakFourierSeq}.
By the correctness proof of Theorem \ref{thm:alg:WeakFourierSeqTC}, $G_i(x,y)\in\Q[y]$ or
\begin{align*}
    G_i(x,y)=a_{in_i}(y)x^{n_i}+\sum_{j=0}^{n_{i}-1}\frac{a_{ij}(y)}{(1+y^2)^{m_{ij}}}x^{j},%+\frac{a_{i0}(y)}{(1+y^2)^{m_{i0}}},
\end{align*}
where $n_i=\deg(G_i,x)\ge1$, $a_{in_i}(y)\in\Q[y]~(1\le i\le k)$ and $m_{ij}\in\N~(0\le j\le n_{i}-1)$.
For $i=1,\ldots,k$, let $m_i:=\max(m_{ij},0\le j\le n_i-1)$ and
\begin{align*}
F_i:=
\left\{
\begin{array}{cc}
G_i, & G_i\in\Q[y],\\
(1+y^2)^{m_{i}}G_i,     &  {\rm otherwise}.
\end{array}
\right.
\end{align*}
We have $F_i\in\Q[x,y]$, and $F_i(r\pi+\arctan{y},y)$ has the same signs and real roots as $G_i(r\pi+\arctan{y},y)$ on $\R$.
Thus, we consider $F_i$ instead of $G_i$ in the next subsection.
%is also a weak Fourier sequence for $G(r\pi+\arctan{y},y)$.
\end{remark}

\subsection{Isolating the roots}\label{subsec:IsoRoot}
Recall that the goal of Section \ref{sec:IBR} is to isolate the roots of the following equation: 
\begin{align}\label{meq:boudedeq1_9}
    g(x,\tan{x}),~x\in(k\pi-\frac{\pi}{2},k\pi+\frac{\pi}{2}),~{\rm where}~k\in\Z.
\end{align}

\subsubsection{The algorithm}
Given $g(x,y)\in\Q[x,y]\setminus\{0\}$ and $k\in\Z$,
% Let $G(x,y)\in\Q[x,y]$ be an irreducible polynomial and $r\in\{k,k+\frac{1}{4}\mid k\in\Z\}$.
%Inspired by \cite[Algorithm 47]{strzebonski2012real}, 
we propose Algorithm \ref{alg:BoundRSI} to isolate the real roots of Eq. \eqref{meq:boudedeq1_9}.
% \begin{align}%\label{meq:boudedeq1_8}
%     g(x,\tan{x}),~x\in(k\pi-\frac{\pi}{2},k\pi+\frac{\pi}{2}).
% \end{align}
% Let $y:=\tan{x}$. It is equivalent to
% \begin{align}%\label{meq:boudedeq1_8}
%     G(r\pi+\arctan{y},y),~y\in(0,1).
% \end{align}

The process of Algorithm \ref{alg:BoundRSI} is as follows.
We first decide whether $k\pi$, $-\frac{\pi}{4}+k\pi$ or $\frac{\pi}{4}+k\pi$ is a root of $g(x,\tan{x})$ by Lemma \ref{lemma:piRealRoot}.
Then, we compute all irreducible factors $g_1,\ldots,g_m$ of $g(x,y)$ in $\Q[x,y]$.
For every $g_i(x,\tan{x})$, we only need to isolate the real roots of it in four open intervals, i.e., $(k\pi-\frac{\pi}{2},k\pi-\frac{\pi}{4})$, $(k\pi-\frac{\pi}{4},k\pi)$, $(k\pi,k\pi+\frac{\pi}{4})$ and $(k\pi+\frac{\pi}{4},k\pi+\frac{\pi}{2})$.
If $g_i$ is a polynomial in $\Q[x]$, it is easy to deal with (there are many methods to isolate the real roots of univariate polynomials).
%, see \textcolor{red}{?} for example).
Otherwise, we have $\deg(g_i,y)\ge1$. 
Let $g_{i}^{(1)}(x,y):=g_{i}(-x,-y)$.
It is easy to check that isolating the real roots of $g_i(x,\tan{x})$ in the first interval (\emph{resp.}, the second interval) is equivalent to isolating those of $g_{i}^{(1)}(x,\tan{x})$ in $(-k\pi+\frac{\pi}{4},-k\pi+\frac{\pi}{2})$ (\emph{resp.}, $(-k\pi,-k\pi+\frac{\pi}{4})$).
Note that these four cases can all be reduced to the problem of isolating the real roots of $G(x,\tan{x})$ on $(r\pi,r\pi+\frac{\pi}{4})$, where $G\in\{g_i,g_{i}^{(1)}\}$ is a rational bivariate irreducible polynomial with $\deg(G,y)\ge1$ and $r\in\{k_0,k_0+\frac{\pi}{4}\}~(k_0\in\Z)$.  
And, Algorithm \ref{alg:SubIBR} can solve such problem, which we will explain in detail in the next subsection. Finally, in Algorithm \ref{alg:AlgDerBound} the isolating intervals obtained from each irreducible factor $g_i$ are refined so that they do not intersect. This is by using Remark \ref{remark:bisect} and the fact that the roots in them are all distinct simple roots (Prop. \ref{prop:multiplicity-one}--\ref{proposition:nocommonroot}).

\begin{algorithm}[!ht]
\scriptsize
\DontPrintSemicolon
\LinesNumbered
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{
$g(x,y)$, a polynomial in $\Q[x,y]\setminus\{0\}$\\
$k$, an integer
%$\varepsilon$, a positive rational number that specifies the maximal length of isolating intervals
    %such that $k^{-}\le k\le k^{+}$ (see \eqref{eq:boudedeq1})
}
\Output{$ans$, a set of pairwise disjoint isolating intervals of real roots of $g(x,\tan{x})$ in $(k\pi-\frac{\pi}{2},k\pi+\frac{\pi}{2})$ 
}
\caption{{\bf IsolatingBoundedRoots}}\label{alg:BoundRSI}
\BlankLine
$ans\leftarrow\emptyset$\;
If $g(k\pi,0)=0$, then $ans\leftarrow ans\cup\{[k\pi,k\pi]\}$\;
If $g(-\frac{\pi}{4}+k\pi,-1)=0$, then $ans\leftarrow ans\cup\{[-\frac{\pi}{4}+k\pi,-\frac{\pi}{4}+k\pi]\}$\;
If $g(\frac{\pi}{4}+k\pi,1)=0$, then $ans\leftarrow ans\cup\{[\frac{\pi}{4}+k\pi,\frac{\pi}{4}+k\pi]\}$\;
$g_1,\ldots,g_m\leftarrow$ all irreducible factors of $g(x,y)$ in $\Q[x,y]$\;
\For{$i$ from $1$ to $m$}
{
\eIf{$g_i$ is a polynomial in $\Q[x]$}
{$S\leftarrow$ a set of isolating intervals of real roots of $g_i(x)$ in $(k\pi-\frac{\pi}{2},k\pi+\frac{\pi}{2})\setminus\{k\pi,-\frac{\pi}{4}+k\pi,\frac{\pi}{4}+k\pi\}$\;
$ans\leftarrow ans\cup S$\;
}
{
let $g_{i}^{(1)}\in\Q[x,y]$ such that $g_{i}^{(1)}(x,y)=g_{i}(-x,-y)$\;
$S_1\leftarrow{\bf SubIBR}(g_{i}^{(1)},-k+\frac{1}{4})$\;
$S_2\leftarrow{\bf SubIBR}(g_{i}^{(1)},-k)$\;
$S_3\leftarrow{\bf SubIBR}(g_{i},k)$\;
$S_4\leftarrow{\bf SubIBR}(g_{i},k+\frac{1}{4})$\;
$ans\leftarrow ans\cup\{(-b,-a)\mid (a,b)\in S_1\cup S_2\}\cup S_3\cup S_4$\;
}
}
Refine the intervals obtained in the loop above such that they do not intersect.\;
\Return{$ans$}\;
\end{algorithm}

\begin{comment}
Let $x_1:=x-k\pi$.
It is equivalent to isolating the real roots of $g_i(x_{1}+k\pi,\tan{x_1})$ in $(-\frac{\pi}{2},-\frac{\pi}{4})$, $(-\frac{\pi}{4},0)$, $(0,\frac{\pi}{4})$ and $(\frac{\pi}{4},\frac{\pi}{2})$.
For the first, the second and the fourth case, we can transform $g_i$ to some bivariate rational polynomial $\tilde{g_i}$ and we only need to consider the real roots of $\tilde{g_i}$ in $(0,\frac{\pi}{4})$.
Take the first case for example.
Let $x_2:=-x_{1}$ and $g_{i}^{(1)}:=g_{i}(-x,-y)$. 
It is easy to check that solving $g_i(x_1+k\pi,\tan{x_1})$ where $x_1\in(-\frac{\pi}{2},-\frac{\pi}{4})$ is equivalent to solving $g_i^{(1)}(x_2-k\pi,\tan{x_2})$ where $x_2\in(\frac{\pi}{4},\frac{\pi}{2})$.
Let $x_3:=x_2-\frac{\pi}{4}$, then $x_3\in(0,\frac{\pi}{4})$. Note that $\tan(x_3+\frac{\pi}{4})=\frac{1+\tan{x_3}}{1-\tan{x_3}}$ and $1-\tan{x_3}>0$.
Then, let $g_{i}^{(2)}\in\Q[x,y]$ be the product of $g_{i}^{(1)}(x,\frac{1+y}{1-y})$ and the common denominator of $g_{i}^{(1)}(x,\frac{1+y}{1-y})$, and thus it becomes solving $g_{i}^{(2)}(x_3+(-k+\frac{1}{4})\pi,\tan{x_3})$ where $x_3\in(0,\frac{\pi}{4})$.
By Algorithm \ref{alg:SubIBR}, we can isolate the real roots of $g_{i}^{(2)}(x_3+(-k+\frac{1}{4})\pi,\tan{x_3})$ in  $(0,\frac{\pi}{4})$.
Remark that $x_3=-x+k\pi-\frac{\pi}{4}$.
If $(a,b)$ is an isolating interval of $g_{i}^{(2)}(x_2+(-k+\frac{1}{4})\pi,\tan{x_2})$ in $(0,\frac{\pi}{4})$, it is obvious that $(-b+k\pi-\frac{\pi}{4},-a+k\pi-\frac{\pi}{4})$ is an isolating interval of $g_i(x,\tan{x})$ in $(k\pi-\frac{\pi}{2},k\pi-\frac{\pi}{4})$.
\end{comment}

\subsubsection{Sub-algorithms}
Let $g(x,y)$ be an irreducible polynomial in $\Q[x,y]$ with $\deg(g,y)\ge1$ and $r\in\{k,k+\frac{1}{4}\}$ where $k\in\Z$. 
% We use \cite[Algorithm 47]{strzebonski2012real}, i.e. Algorithm \ref{alg:SubIBR} in the paper to isolate the real roots of $g(r\pi+x,\tan{x})$ in $(0,\frac{\pi}{4})$.
According to the frame of \cite[Algorithm 47]{strzebonski2012real}, Algorithm \ref{alg:SubIBR} is proposed to isolate the real roots of $g(x,\tan{x})$ in $(r\pi,r\pi+\frac{\pi}{4})$.
It is worth noting that \cite[Algorithm 47]{strzebonski2012real} and Algorithm \ref{alg:SubIBR} are not the same.
Some steps are added, and some steps are skipped or implemented in another way.
% We skip some steps, add some steps and implement some steps in another way. 
%of it.

% Let us recall the frame of \cite[Algorithm 47]{strzebonski2012real} first.
The algorithm \cite[Algorithm 47]{strzebonski2012real} can be used to isolate the real roots of an exp-log-arctan function $w(y)$ in an open interval $(a,b)$, where $a,b$ are rational numbers and $(a,b)$ are contained in the domain of $w(y)$.
% Let $y:=\tan{x}$.
% Our problem becomes solving $w(y):=g(r\pi+\arctan{y},y)$ in $(0,1)$, and thus we can use the frame of \cite[Algorithm 47]{strzebonski2012real} to deal with it.
Let us review the frame of the algorithm.
%(also see Algorithm \ref{alg:SubIBR}).
% The frame of the algorithm is as follows.
We need to compute a weak Fourier sequence $w_1,\ldots,w_k$ for $w(y)$ on $(a,b)$ first.
Let $ans$ be a set of computed isolating intervals of $w(y)$ (initialized as $\emptyset$), and $stack$ be a stack of triples $(c,d,m)$ such that $c<d$ are rational numbers and $w_m$ has a constant nonzero sign in $(c,d)$ (initialized as $(a,b,k)$).
In each loop step, we pick a triple $(c,d,m)$ from $stack$ and compute the difference value $\sgc_{1,m}(c^{+})-\sgc_{1,m}(d^{-})$ by \cite[Algorithm 44]{strzebonski2012real}, 
%(i.e. Algorithm \ref{alg:SGC} in the paper), 
until $stack$ is empty.
\begin{enumerate}
    \item If the value equals $0$, by Theorem \ref{thm:WeakFourierSeq}, $w(y)$ has no roots on $(c,d)$. So, we continue for the next loop step. 
    \item If the value equals $1$, by Theorem \ref{thm:WeakFourierSeq}, $w(y)$ has exactly one simple root on $(c,d)$. We add $(c,d)$ to $ans$.
    \item Otherwise, let $\ell$ be the smallest element of $\{i\mid 2\le i\le m \;{\rm and}\; \sgc_{i,m}(c^{+})\allowbreak-\sgc_{i,m}(d^{-})=1\}$.
    By Theorem \ref{thm:WeakFourierSeq}, $w_{\ell}(y)$ has exactly one simple root $sr$ on $(c,d)$.
    \begin{enumerate}
        \item If $sr$ is a root of $w(y)$, find two rational numbers $u,v$ such that $c<u<sr<v<d$ and $w(y)$ has only one root $sr$ in $[u,v]$
    (recall that by Lemma \ref{lemma:NoLimit}, we can find such $u,v$).
    Add $(u,v)$ to $ans$, and add $(c,u,\ell)$, $(v,d,\ell)$ to $stack$.
    \item If $sr$ is not a root of $w(y)$. Find two rational numbers $u,v$ such that $c<u<sr<v<d$ and $w(y)$ has no roots in $[u,v]$.     
    Add $(c,u,\ell)$ and $(v,d,\ell)$ to $stack$.
    \end{enumerate}
\end{enumerate}

\begin{comment}
Back to Algorithm \ref{alg:SubIBR}, we will explain some differences between the two algorithms and some implementation details in the following.

Instead of using \cite[Algorithm 40]{strzebonski2012real} to compute a semi-Fourier sequence, we directly compute a weak Fourier sequence $w_1=G_1(r\pi+\arctan{y},y),\ldots,w_k=G_k(r\pi+\arctan{y},y)$, where $G_i\in\Q(y)[x]$, for $w(y)$ on $(0,1)$ by Algorithm \ref{alg:WeakFourierSeq}.
Recall Remark \ref{remark:PolyWeakFourierSeq}.
We have $G_i\in\Q[x,y]$ in fact (see Algorithm \ref{alg:SubIBR}-Line \ref{algline:SubIBR-weakFseq}).

{\bf How to compute $\sgc_{i,m}(c^{+})$ or $\sgc_{i,m}(c^{-})$, where $c\in\Q$ and $1\le i\le m$?} We use Algorithm \cite[Algorithm 44]{strzebonski2012real}, i.e. Algorithm \ref{alg:SGC} in the paper, to compute it.
\end{comment}
\begin{comment}
\begin{definition}
A \emph{root constant} is an expression $\Root(G,a,b)$, where $G\in\R[x]$, $a<b$ are rational numbers such that $(a,b)$ is contained in the domain of $G$ and $G$ has the only root in $(a,b)$. $\Root(G,a,b)$ represents the only root of $G$ in $(a,b)$.
\end{definition}

\begin{lemma}
Let $G(x,y)$ be an irreducible polynomial in $\Q[x,y]$ and $r\in\Q$.
Then, $w(y)=G(r\pi+\arctan{y},y)$ has no multiple roots in $(0,1)$.
\end{lemma}
\end{comment}
\begin{comment}
\begin{lemma}
Let $w_1(y)=G_1(r\pi+\arctan{y},y),\ldots,w_k(y)=G_k(r\pi+\arctan{y},y)$ be a weak Fourier sequence for $w_1(y)$, where $G_i\in\Q[x,y]$ (see Remark \ref{remark:PolyWeakFourierSeq}) and $\Root(w_{\ell},c,d)~(l\ge2)$ be a simple root.
Then, there exists $u,v\in\Q$ such that $c<u<\Root(w_{\ell},c,d)<v<d$ and $\sgc_{1,l}$
\end{lemma}
\end{comment}

Before we explain Algorithm \ref{alg:SubIBR}, we first define a map $\varphi$ and introduce Lemma \ref{lemma:mappingirre} and Lemma \ref{lemma:NoCommonRoot}.
The map $\varphi:\;{\mathbb Q}[x,y]\to{\mathbb Q}[x,y_1]$  is defined as
\begin{align}\label{eq:def-map1}
\varphi(g(x,y))=g(x,\frac{1+y_1}{1-y_1})\cdot(1-y_1)^{\deg(g,y)}.
\end{align}

\begin{lemma}\label{lemma:mappingirre}
If $g$ is an irreducible polynomial in $\Q[x,y]\setminus\{c(y+1)\mid c\ne0\}$, then $\varphi(g)$ is an irreducible polynomial in $\Q[x,y_1]$.
% We have the following statements:
% \begin{enumerate}[(a)]
%     \item $\psi(\varphi(g))=g$,\label{item:lemma:mappingirre1}
%     \item $\varphi(g)$ is an irreducible polynomial in $\Q[x,y_1]$.\label{item:lemma:mappingirre2}
% \end{enumerate}
\end{lemma}
\begin{proof}
Since $\deg(g(x,2y-1),y)=\deg(g(x,y),y)$, $\varphi(g)=\mathcal{R}(g(x,2y-1))|_{y=1-y_1}$ with $\mathcal{R}$ in Definition \ref{definition:recip}. Now that $g(x,y)\neq c(y+1)$ for any nonzero $c\in\Q$, $g(x,2y-1)\neq cy$ for any nonzero $c\in\Q$. Moreover, $g(x,2y-1)$ is irreducible since $g(x,y)$ is. By Proposition \ref{proposition:RkeepIrr}, $\mathcal{R}(g(x,2y-1))$ is irreducible. Thus so is $\varphi(g)=\mathcal{R}(g(x,2y-1))|_{y=1-y_1}$.
\end{proof}
The following lemma is similar to \cite[Lemma 3.2]{chen2022automated} and \cite[Theorem 7]{mccallum2012deciding}.% The proof given below is almost the same to the proof of the latter:
\begin{lemma}\label{lemma:NoCommonRoot}
Let $F_1,F_2\in\Q[x,y]$, $k\in\Z$ and $r\in\{k,k+\frac{1}{4}\}$.
If ${\gcd}(F_1,F_2)=1$, then $F_1(r\pi+\arctan{y},y)$ and $F_2(r\pi+\arctan{y},y)$ have no common real roots in $(0,1)$.
\end{lemma}
\begin{proof}
Replacing those ``$p,q$" in the proof of \cite[Theorem 7]{mccallum2012deciding} by $F_1$ and $F_2$ in this lemma, those ``$f^*(x),g^*(x)$" therein by $F_1(r\pi+\arctan{y},y)$ and $F_2(r\pi+\arctan{y},y)$, and the function ``\text{trans}" therein by the function $r\pi+\arctan$, we see that: If $\beta\in(0,1)$ is a common root of $F_1(r\pi+\arctan{y},y)$ and $F_2(r\pi+\arctan{y},y)$, then both $\beta$ and $\alpha=r\pi+\arctan{\beta}$ would be algebraic, which contradicts Claim \ref{claim:atleastonetrans} below.
% We only need to prove that $F_1(x,y)=0$, $F_2(x,y)=0$ and $x=r\pi+\arctan{y}$ have no common real roots on $(0,1)$.
% Assume that $y_0\in(0,1)$ is a common real root.
% Let $x_0:=r\pi+\arctan{y_0}$.
% Then, $(x_0,y_0)$ is a solution of $F_1(x,y)=0$, $F_2(x,y)=0$.
% Note that since $\deg(F_1,y)\ge1$, $\deg(F_2,y)\ge1$ and ${\gcd}(F_1,F_2)=1$, by \cite[Prop.1, Sec.6, Chap.3]{cox2013ideals}, $\res(F_1,F_2,y)$ is not the zero polynomial.
% So, $x_0$ is a root of $\res(F_1,F_2,y)$, and thus $x_0$ an algebraic number.
% We also note that at least one of $F_1(x_0,y)$ and $F_2(x_0,y)$ is not zero, since ${\gcd}(F_1,F_2)=1$.
% So, $y_0$ is also an algebraic number. This results in a contradiction according to Claim \ref{claim:atleastonetrans}.
%In fact, we have the claim below. Then, the case that $x_0$ and $y_0$ are both algebraic numbers makes a contradiction.
\end{proof}
\begin{claim}\label{claim:atleastonetrans}
%\textcolor{blue}{
For any $y\in(0,1)$, at least one of $r\pi+\arctan{y}$ and $y$ is transcendental. %(proof re-organized)}
\end{claim}
\begin{proof}
Note that \[
\tan(r\pi+\arctan y)=\left\{
\begin{array}{ccl}\vspace{2mm}
     y,& \text{ if } &r=k\in\mathbb{Z},\\
     \frac{1+y}{1-y},& \text{ if }  &r=k+\frac{1}{4}\in\mathbb{Z}+\frac{1}{4}.
\end{array}
\right.
\]
Suppose $y$ is algebraic, then $\tan(r\pi+\arctan y)$ is also algebraic in either case. Since neither $y$ nor $(1+y)/(1-y)$ is zero, $r\pi+\arctan y\neq0$. Moreover, it is transcendental by Theorem \ref{thm:BothAlgeNum}.
% If $r=k$, assume that $k\pi+\arctan{y}$ and $y$ are both algebraic numbers. 
% Note that $\tan(k\pi+\arctan{y})=y$. Then, by Theorem \ref{thm:BothAlgeNum}, we have $y=0$, which makes a contradiction.
% If $r=k+\frac{1}{4}$, assume that $k\pi+\frac{\pi}{4}+\arctan{y}$ and $y$ are both algebraic numbers.
% Let $x:=k\pi+\frac{\pi}{4}+\arctan{y}$.
% Then, $\tan{x}=\frac{1+y}{1-y}$.
% Let $z:=\tan{x}$.
% Then, we have $(y-1)z+y+1=0$.
% Since $y$ is an algebraic number, $z$ is also an algebraic number.
% Since $x$ and $z$ are both algebraic numbers, by Theorem \ref{thm:BothAlgeNum}, we have $z=0$.
% Then, $y=-1$, which makes a contradiction.
\end{proof}
\begin{remark}\label{remark:bisect}
Suppose $h(x_1,x_2)=\sum_{i=0}^{\deg(h,x_1)}c_i(x_2)x_1^i\in\mathbb{Q}[x_1,x_2]$. For any $y\in(0,1)\cap\mathbb{Q}$, $r\pi+\arctan y$ is transcendental. Thus $h(r\pi+\arctan y,y)=0$ iff $c_i(y)=0$ for all $i$. We can therefore decide whether $h(r\pi+\arctan y,y)$ is zero for given $y\in(0,1)\cap\mathbb{Q}$. If it is nonzero, we can further compute its sign by approximating it more accurately. More generally, if $\phi$ is a real function $($\emph{e.g.}, $\phi=\tan)$ such that $\phi(y)$ is transcendental for any nonzero rational $y$ in its domain, then we can decide whether $h(\phi(y),y)$ is zero, and compute its sign whenever it is not zero.
\end{remark}
\begin{comment}
\begin{lemma}\label{lemma:NoCommonRootPre}
Let $k\in\Z$ and $r\in\{k,k+\frac{1}{4}\}$.
For any $y\in(0,1)$, at least one of $r\pi+\arctan{y}$ and $y$ is an  transcendental number.
\end{lemma}
\begin{proof}
If $r=k$, assume that $k\pi+\arctan{y}$ and $y$ are both algebraic numbers. 
Note that $\tan(k\pi+\arctan{y})=y$. Then, by Theorem \ref{thm:BothAlgeNum}, we have $y=0$, which makes a contradiction.

If $r=k+\frac{1}{4}$, assume that $k\pi+\frac{\pi}{4}+\arctan{y}$ and $y$ are both algebraic numbers.
Let $x:=k\pi+\frac{\pi}{4}+\arctan{y}$.
Then, $\tan{x}=\frac{1+y}{1-y}$.
Let $z:=\tan{x}$.
Then, we have $(y-1)z+y+1=0$.
Since $y$ is an algebraic number, $z$ is also an algebraic number.
Since $x$ and $z$ are both algebraic numbers, by Theorem \ref{thm:BothAlgeNum}, we have $z=0$.
Then, $y=-1$, which makes a contradiction.
\end{proof}
\end{comment}

Recall that our goal is to isolate the real roots of $g(x,\tan{x})$ in $(r\pi,r\pi+\frac{\pi}{4})$, where $g$ is an irreducible polynomial in $\Q[x,y]$ with $\deg(g,y)\ge1$ and $r\in\{k,k+\frac{1}{4}\}~(k\in\Z)$. 
The process of Algorithm \ref{alg:SubIBR} is as follows.
If $g=y+1$, then $\tan{x}+1$ has no roots on $(r\pi,r\pi+\frac{\pi}{4})$, and thus return $\emptyset$.
Otherwise, let $F_1:=g$ when $r=k$, and $F_1:=\varphi(g)$ when $r=k+\frac{1}{4}$.
It is not difficult to check that our goal is equivalent to solving $F_1(x+r\pi,\tan{x})$ on $(0,\frac{\pi}{4})$.
Let $y:=\tan{x}$.
We only need to solve $F_1(r\pi+\arctan{y},y)$ on $(0,1)$.
Recall Remark \ref{remark:PolyWeakFourierSeq}.
We can compute a weak Fourier sequence
\begin{align}\label{eq:ComputeFourierSeq}
    w_1=F_1(r\pi+\arctan{y},y),\ldots,w_k=F_k(r\pi+\arctan{y},y)~{\rm on}~(0,1),
\end{align}
where $F_i\in\Q[x,y]$.
Thus, the frame of \cite[Algorithm 47]{strzebonski2012real} can be used.
However, there are two main differences between \cite[Algorithm 47]{strzebonski2012real} and Algorithm \ref{alg:SubIBR}.

\begin{comment}
First, we use Algorithm \ref{alg:WeakFourierSeq} to compute a weak Fourier sequence 
\begin{align}\label{eq:ComputeFourierSeq}
    w_1=G_1(r\pi+\arctan{y},y),\ldots,w_k=G_k(r\pi+\arctan{y},y),
\end{align}
where $G_i\in\Q[x,y]$, for $G_1(r\pi+\arctan{y},y)$ on $(0,1)$ (see Line \ref{algline:SubIBR-weakFseq}), instead of \cite[Algorithm 40]{strzebonski2012real}.
Although \cite[Algorithm 40]{strzebonski2012real} is more general and can also be used to compute a weak Fourier sequence for $G_1(r\pi+\arctan{y},y)$, Algorithm \ref{alg:WeakFourierSeq} is better since it is proposed particularly for our purpose. 
\end{comment}

First, when $w_{\ell}$ has exactly one simple root $sr$ on $(c,d)$ (see Line \ref{algline:SubIBR-sr}),
we propose a new method to decide whether $sr$ is a root of $w_1$. %where $sr$ is the only root of $w_{\ell}$ on $(c,d)$ (see Line \ref{algline:SubIBR-sr}). 
If $F_{\ell}=QF_1~(Q\in\Q[y])$ holds and $Q$ has no roots on $(c,d)$, by \eqref{eq:ComputeFourierSeq}, $sr$ is the only root of $w_1$ on $(c,d)$.
If $F_{\ell}=QF_1$ holds and $Q$ has roots on $(c,d)$, then it is clear that $w_1$ has no roots on $(c,d)$.
If $F_{\ell}=QF_1$ does not hold, then $sr$ is not a root of $w_1$.
This method is correct: By Lemma \ref{lemma:mappingirre}, $F_1$ is an irreducible polynomial.
If $F_1\mid F_{\ell}$, we have $\deg(F_1,x)\le\deg(F_{\ell},x)$.
Then, by Lemma \ref{lemma:pseudoproperty}, $\deg(F_1,x)=\deg(F_{\ell},x)$.
So, $Q$ is a polynomial in $\Q[y]$.
Otherwise, ${\gcd}(F_1,F_{\ell})=1$. Then, by Lemma \ref{lemma:NoCommonRoot}, $sr$ is not a root of $w_1$.

Second, if $sr$ is not a root of $w_1$, we find two rational numbers $u,v$ such that $c\leq u<sr<v\leq d$ and $w_1$ has no roots in $[u,v]$ by Algorithm \ref{alg:RationalEndpoint} (see Line \ref{algline:SubIBR-RationalEP} of Algorithm \ref{alg:SubIBR}), instead of by \cite[Algorithm 45]{strzebonski2012real}. The process of Algorithm \ref{alg:RationalEndpoint} is as follows: Let $n:=1$.
While $n\ge1$, we compute an upper limit polynomial $W_{\max,n}\in\Q[y]$ and a lower limit polynomial $W_{\min,n}\in\Q[y]$ for $w_1(y)$ by two steps.
Since $w_1=F_1(r\pi+\arctan{y},y)$, we first estimate $\arctan{y}$ through Taylor series, and $T_{\max}(n,w_1),T_{\min}(n,w_1)\in\Q[\pi][y]$ are computed by \cite[Def. 3.1]{chen2020automated}.
Then, we use a bounded interval with rational endpoints to estimate $\pi$ in $T_{\max}(n,w_1)$ and $T_{\min}(n,w_1)$, and the polynomials $W_{\max,n},W_{\min,n}\in\Q[y]$ are computed by \cite[Def. 3.1]{xia2006real}.
% (since $w_1=G_1(r\pi+\arctan{y},y)$, we estimate $\arctan{y}$ and $\pi$ by \cite[Def. 3.1]{chen2020automated} and \cite[Def. 3.1]{xia2006real}, respectively).
Let $q:=\frac{c+d}{2}$.
If $W_{\max,n}$ has no roots on $[c,d]$ and $W_{\max,n}(q)<0$, or if $W_{\min,n}$ has no roots on $[c,d]$ and $W_{\min,n}(q)>0$, then $w_1$ has no roots on $[c,d]$.
Otherwise, increase $n$ by $1$.
Since $w_{\ell}$ has exactly one simple root $sr$ on $(c,d)$, we use a bisection method based on Remark \ref{remark:bisect} to find the half open interval where $sr$ is.
Update $(c,d)$ as the half interval and go for the next loop step.
% We will explain the termination of Algorithm \ref{alg:RationalEndpoint}.
Remark that if the interval $(c,d)$ is small enough and the upper (lower) limit polynomial is close enough, Algorithm \ref{alg:RationalEndpoint} terminates by Lemma \ref{lemma:NoLimit}.

\begin{algorithm}[!t]
\scriptsize
\DontPrintSemicolon
\LinesNumbered
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{
$g(x,y)$, an irreducible polynomial in $\Q[x,y]$ with $\deg(g,y)\ge1$\\
$r$, $r\in\{k,k+\frac{1}{4}\}$ where $k\in\Z$
}
\Output{$ans$, a set of isolating intervals of real roots of $g(x,\tan{x})$ in $(r\pi,r\pi+\frac{\pi}{4})$ 
}
\caption{{\bf SubIBR} 
}\label{alg:SubIBR}
\BlankLine
{\bf if} $g=y+1$, {\bf then} {\bf return} $\emptyset$\;
\eIf{$r=k$}
{$F_1\leftarrow g$}
{$F_1\leftarrow g(x,\frac{1+y}{1-y})\cdot(1-y)^{\deg(g,y)}$\;}
let $w_1=F_1(r\pi+\arctan{y},y),\ldots,w_k=F_k(r\pi+\arctan{y},y)$, where $F_i\in\Q[x,y]$, be the sequence in Remark \ref{remark:PolyWeakFourierSeq}\label{algline:SubIBR-weakFseq}\;
$ans\leftarrow\emptyset$\;
$stack\leftarrow\{(0,1,k)\}$\;
\While{$stack\ne\emptyset$}
{
$(c,d,m)\leftarrow First(stack),\;stack\leftarrow Rest(stack)$\;
$sgc\leftarrow\sgc_{1,m}(c^{+})-\sgc_{1,m}(d^{-})$\;
{\bf if} $sgc=0$, {\bf then} continue\;
\If{$sgc=1$}{$ans\leftarrow ans\cup\{(r\pi+\arctan{c},r\pi+\arctan{d})\}$\; continue\;}
$\ell\leftarrow\min\;\{i\mid 2\le i\le m,~\sgc_{i,m}(c^{+})-\sgc_{i,m}(d^{-})=1\}$\;
$sr\leftarrow\Root(w_{\ell},c,d)$\label{algline:SubIBR-sr}\;
By Theorem \ref{thm:WeakFourierSeq}, $w_{\ell}$ has exactly one simple root $sr$ in $(c,d)$.
We use the notation $\Root(w_{\ell},c,d)$ to represent the only simple root of $w_{\ell}$ in $(c,d)$.\;
\eIf{$F_{\ell}=QF_1$ where $Q\in\Q[y]$\label{algline:SubIBR-wheHold}}
{
\eIf{$Q$ has no real roots on $(c,d)$}
{$ans\leftarrow ans\cup\{(r\pi+\arctan{c},r\pi+\arctan{d})\}$}
{continue}
}
{
$u,v\leftarrow{\bf RationalEndpoint}(w_1,w_{\ell},sr)$\label{algline:SubIBR-RationalEP}\;
add $(c,u,\ell)$ and $(v,d,\ell)$ to $stack$\;
}
}
\Return{$ans$}
\end{algorithm}

\begin{algorithm}[htbp]
\scriptsize
\DontPrintSemicolon
\LinesNumbered
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{
% \begin{itemize}
    $w_1(y)=F_1(r\pi+\arctan{y},y)$, where $F_1(x,y)\in\Q[x,y]$, $r\in\Q$\\
    $w_{\ell}(y)=F_{\ell}(r\pi+\arctan{y},y)$, where $F_{\ell}(x,y)\in\Q[x,y]$\\
    $sr=\Root(w_{\ell},c,d)$, $w_{\ell}$ has exactly one simple root $sr$ in $(c,d)$ and $w_{1}(sr)\ne0$
% \end{itemize}
}
\Output{two rational numbers $u$ and $v$ $(c\leq u<sr<v\leq d)$ such that $w_{1}$ has no roots on $[u,v]$
}
\caption{{\bf RationalEndpoint}}\label{alg:RationalEndpoint}
\BlankLine
$n\leftarrow1$\;
\While{$n\ge1$}{
Compute an upper limit polynomial $W_{\max,n}\in\Q[y]$ and a lower limit polynomial $W_{\min,n}\in\Q[y]$ for $w_1(y)$\;
% \textcolor{blue}{($\arctan{y}$: Chen Shiping 1, $\pi$: series + Zhang Ting)}
% We need a upper/lower limit polynomial which contains the series of $\pi$ and $\arctan{y}$ together
$q\leftarrow\frac{c+d}{2}$\;
\eIf{$(W_{\max,n}$ has no roots on $[c,d]$ and $W_{\max,n}(q)<0)$
{\bf or} \\$\quad\,(W_{\min,n}$ has no roots on $[c,d]$ and $W_{\min,n}(q)>0)$
}
{\Return{$c,d$}}
{
 $n\leftarrow n+1$\;
%$\textcolor{blue}{for deciding whether $w_\ell(q)=0$, is it necessary to use the claim in the proof of Lemma \ref{lemma:NoCommonRoot}? Tianqi: Yes. If $F_{\ell}(x,q)\equiv0$, then $q$ is a root of $w_{\ell}$.
% Otherwise, by the claim, $q$ is not a root of $w_{\ell}$.
% }\;
% \eIf{$\sign(f_i({\tilde c})f_i(q))=-1$}
% {${\tilde d}\leftarrow q$}
% {${\tilde c}\leftarrow q$}
\uIf{$w_{\ell}(q)=0$}
{$c\leftarrow \frac{63q+c}{64},\;d\leftarrow\frac{63q+d}{64}$}
\uElseIf{$\sign(w_{\ell}(c)w_{\ell}(q))=-1$}
{$d\leftarrow q$}
\Else{$c\leftarrow q$}
}
}
\end{algorithm}

% It remains to prove Lemma \ref{lemma:mappingirre}.
% % and Lemma \ref{lemma:NoCommonRoot}.
% In order to prove Lemma \ref{lemma:mappingirre}, we define a homomorphism and prepare Lemma \ref{lemma:mappingdeg=} and Lemma \ref{lemma:mappingNotfactor}.
% % In order to prove Lemma \ref{lemma:NoCommonRoot}, we prepare Lemma \ref{lemma:NoCommonRootPre}.
% %Let $g\in\Q[x,y]$ and $G\in\Q[x,y_1]$. 
% The homomorphism is defined as $\psi:\;{\mathbb Q}[x,y_1]\to{\mathbb Q}[x,y]$ such that
% \begin{align}\label{eq:def-map2}
% \psi(G(x,y_1))=G(x,\frac{y-1}{y+1})\cdot(\frac{y+1}{2})^{\deg(G,y_1)}.
% \end{align}

% \begin{lemma}\label{lemma:mappingdeg=}
% Let $g$ be an irreducible polynomial in $\Q[x,y]\setminus\{c(y+1)\mid c\ne0\}$
% %with $\deg(g,y)\ge1$ 
% and $G$ be an irreducible polynomial in $\Q[x,y_1]\setminus\{c(y_{1}-1)\mid c\ne0\}$. %with $\deg(G,y_1)\ge1$.
% Then, we have $\deg(\varphi(g),y_1)=\deg(g,y)$ and $\deg(\psi(G))=\deg(G)$.
% \end{lemma}
% \begin{proof}
% We prove $\deg(\psi(G),y)=\deg(G,y_1)$ first. 
% %since the proof of $\deg(\psi(G),y)\allowbreak=\deg(G,y_1)$ is similar.
% If $\deg(G,y_1)=0$, we have $\psi(G)=G$.
% If $\deg(G,y_1)=d\ge1$, suppose that  
% \begin{align}\label{eq:lemma:mappingdeg=}
%     G(x,y_1)=\sum_{i=0}^{d}a_i(x)y_{1}^{i},~{\rm where}~a_i(x)\in\Q[x].
% \end{align}
% Then,
% \begin{align}
%     \psi(G)&=\sum_{i=0}^{d}a_i(x)(\frac{y-1}{y+1})^{i}(\frac{y+1}{2})^{d}\nonumber\\
%     &=\frac{1}{2^d}\sum_{i=0}^{d}a_i(x)(y-1)^{i}(y+1)^{d-i}\nonumber\\
%     &=\frac{1}{2^d}\left(\sum_{i=0}^{d}a_i(x)\right)y^{d}+\frac{1}{2^d}\sum_{i=0}^{d-1}b_{i}(x)y^{i},%~{\rm where}~b_i\in\Q[x].
% \end{align}
% where $b_i(x)$ is a linear combination of $a_0(x),\ldots,a_d(x)$.
% Assume $\deg(\varphi(G),y)\ne d$.
% Then, 
% %$\sum_{i=0}^{d}(-1)^{d-i}a_i(x)\equiv0$, which means
% $\sum_{i=0}^{d}a_i(x)$ is the zero polynomial.
% So, by \eqref{eq:lemma:mappingdeg=}, $G(x,1)$ is also the zero polynomial, i.e., $y_{1}-1$ is a factor of $G$.
% Since $G$ is irreducible, we have $G=c(y_{1}-1)~(c\ne0)$,
% which causes a contradiction.
% Therefore, $\deg(\psi(G),y)=d$.
% Similarly, we have $\deg(\varphi(g),y_1)=\deg(g,y)$.

% Note that for every $i~(0\le i\le d)$, 
% the coefficient of $\psi(G)$ w.r.t. $y_1^i$ is a linear combination of $a_0(x),\ldots,a_n(x)$.
% So, it is clear that $\deg(\psi(G))=\deg(G)$.
% \end{proof}

% \begin{lemma}\label{lemma:mappingNotfactor}
% For any $g\in\Q[x,y]$, $y_{1}-1$ is not a factor of $\varphi(g)$.
% \end{lemma}
% \begin{proof}
% It is obvious when $\deg(g,y)=0$.
% If $\deg(g,y)=d\ge1$, suppose that $g=\sum_{i=0}^{d}a_i(x)y^i$, where $a_i(x)\in\Q[x]$.
% Recall the definition of $\varphi$ (see \eqref{eq:def-map1}).
% So, 
% \begin{align}\label{eq:lemma:mappingNotfactor}
%     \varphi(g)=a_d(x)(1+y_1)^d+\sum_{i=0}^{d-1}a_{i}(x)(1+y_1)^{i}(1-y_1)^{d-i}.
%     % a_{d-1}(x)(1+y_1)^{d-1}(1-y_1)+\cdots+a_0(x)(1-y_1)^d.
% \end{align}
% Assume that $y_{1}-1$ is a factor of $\varphi(g)$.
% Then, we have $\varphi(g)(x,1)$ is the zero polynomial.
% So, by \eqref{eq:lemma:mappingNotfactor}, $2^{d}a_{d}(x)$ is also the zero polynomial which contradicts the fact that $\deg(g,y)=d$.
% Therefore, $y_1-1$ is not a factor of $\varphi(g)$.
% \end{proof}

% \begin{lemma}\label{lemma:mappingirre}
% Let $g$ be an irreducible polynomial in $\Q[x,y]\setminus\{c(y+1)\mid c\ne0\}$.
% We have the following statements:
% \begin{enumerate}[(a)]
%     \item $\psi(\varphi(g))=g$,\label{item:lemma:mappingirre1}
%     \item $\varphi(g)$ is an irreducible polynomial in $\Q[x,y_1]$.\label{item:lemma:mappingirre2}
% \end{enumerate}
% \end{lemma}
% \noindent{\bf Proof of Lemma \ref{lemma:mappingirre}.}
% %\begin{proof}
% First, we prove that $\psi(\varphi(g))=g$.
% By Lemma \ref{lemma:mappingdeg=}, we have $\deg(\varphi(g),y_1)=\deg(g,y)$.
% Then, it is easy to check that $\psi(\varphi(g))=g$.

% %(\ref{item:lemma:mappingirre2}) 
% Second, we prove that $\varphi(g)$ is irreducible.
% Assume that $\varphi(g)$ is reducible. 
% For simplicity, suppose that 
% \begin{align}\label{eq:lemma:mappingirre1}
%     \varphi(g)=g_{1}g_{2},~{\rm where}~g_1,g_2~{\rm are~ irreducible~polynomials~in}~\Q[x,y_1].
% \end{align}
% Note that by Lemma \ref{lemma:mappingNotfactor}, we have 
% $g_1,g_2\in\Q[x,y_1]\setminus\{c(y_{1}-1)\mid c\ne0\}$.
% By \eqref{eq:lemma:mappingirre1} and by the conclusion in the last paragraph, we have
% $g=\psi(g_1)\psi(g_2)$.
% By Lemma \ref{lemma:mappingdeg=}, for $i=1,2$, $\deg(\psi(g_i))=\deg(g_i)\ge1$.
% So, the equation $g=\psi(g_1)\psi(g_2)$ contradicts the fact that $g$ is irreducible.
% Therefore, $\varphi(g)$ is irreducible.\qed
%\end{proof}

\begin{comment}
\begin{algorithm}[!ht]
% \scriptsize
\DontPrintSemicolon
\LinesNumbered
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{
\begin{itemize}
    \item $c,d$, two rational numbers
    \item $w_i,\ldots,w_m$, a weak Fourier sequence on $(c,d)$
    % $w_i(y)=G_i(r\pi+\arctan{y},y),\ldots,w_m(y)=G_m(r\pi+\arctan{y},y)$ where $G_j\in\Q[x,y]$ and $r\in\Q$, a weak Fourier sequence for $w_i(y)$ on $(c,d)$ 
    %(see Remark \ref{remark:PolyWeakFourierSeq})
    % \item $c$, a rational number
    \item $dir\in\{left,right\}$
\end{itemize}
}
\Output{
$sgc$, if $dir=left$, $sgc$ equals $\sgc_{i,m}(c^{+})$; if $dir=right$, $sgc$ equals $\sgc_{i,m}(d^{-})$
}
\caption{{\bf SGC} \cite[Algorithm 44]{strzebonski2012real}}\label{alg:SGC}
\BlankLine
$s_m\leftarrow\sign(w_m(\frac{c+d}{2}))$\;
{\footnotesize \# Recall Definition \ref{def:WeakFourierSeq}, $w_m(y)\ne0$ for any $y\in(c,d)$. So, $\sign(w_m(y))$ is constant on $(c,d)$.}\;
\eIf{$dir=left$}
{$l_i,\ldots,l_{m-1}\leftarrow\sign(w_i(c^{+})),\ldots,\sign(w_{m-1}(c^{+}))$\;
%{\footnotesize \# If $w_j(c)=0$, then $\sign(w_j(c))=0$.}\;
}
{$l_i,\ldots,l_{m-1}\leftarrow\sign(w_i(d^{-})),\ldots,\sign(w_{m-1}(d^{-}))$}
 %\textcolor{blue}{(write details somewhere)}\;
\For{$j$ {\bf from} $m-1$ {\bf to} $1$}
{If $l_j\ne0$, set $s_j\leftarrow l_j$\;
 If $l_j=0$ and $dir=left$, if $s_{j+1}>0$ set $s_j\leftarrow 1$ and otherwise $s_j\leftarrow -1$\;
 If $l_j=0$ and $dir=right$, if $s_{j+1}>0$ set $s_j\leftarrow -1$ and otherwise $s_j\leftarrow 1$\;
}
\Return{the number of sign changes in the sequence $s_1,\ldots,s_m$}\;
%\textcolor{blue}{\# The correctness of Algorithm \ref{alg:SGC} is guaranteed by Lemma \ref{lemma:NoLimit}}.
\end{algorithm}
\end{comment}
\begin{comment}
\begin{proposition}
If $f(x,y)\in\Q[x,y]\setminus\{0\}$ and $f_1(x,\arctan(x)),\ldots,f_k(x,\arctan(x))$ is a weak Fourier sequence for $f(x,\arctan(x))$ computed by Algorithm \ref{alg:WeakFourierSeq},
then for any nonzero rational number $r$, $f(x,y+r\pi)\in\Q[\pi][x,y]\setminus\{0\}$ and $f_1(x,\arctan(x)+r\pi),\ldots,f_k(x,\arctan(x)+r\pi)$ is a weak Fourier sequence for $f(x,\arctan(x)+r\pi)$.
\end{proposition}
\begin{proof}
It is obvious that $f(x,y+r\pi)\in\Q[\pi][x,y]\setminus\{0\}$.
Note that 
$${\trueder f}(x,\arctan(x)+r\pi)=f'(x,\arctan(x)+r\pi).$$
So, by the correctness proof of Theorem \ref{thm:alg:WeakFourierSeqTC}, $f_1(x,\arctan(x)+r\pi),\ldots,f_k(x,\arctan(x)+r\pi)$ is a weak Fourier sequence for $f(x,\arctan(x)+r\pi)$.
%\qed
\end{proof}
\end{comment}



==> Isolating all the Real Roots of a Trigonometric-Polynomial/fig/e37.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{fig/e37_1.pdf}
    \caption{The figure of the terminal-root-functions of $g$ bounded by $(-\frac{215}{128},-\frac{19}{32}
    )$. 
    The red dotted line and the orange dashed line (which are both vertical) show the graph of the start-point $x=M$ and that of $x=(k'+1/2)\pi$, respectively.
    The two green dotted lines (which are horizontal) show the graphs of $y=-\frac{215}{128}$ and $y=-\frac{19}{32}$.
    When $x>(k'+1/2)\pi$, the terminal-root-functions (plotted as blue curves) are both bounded by the interval $(-\frac{215}{128},-\frac{19}{32}
    )$.
    }
    \label{fig:thm:location-of-the-roots}
\end{figure}


==> Isolating all the Real Roots of a Trigonometric-Polynomial/fig/fig_runtime.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{fig/runtime.pdf}
    \caption{Number of Solved MTPs within Given Time (s: seconds). }
    \label{fig:num-within-time}
\end{figure}


==> Isolating all the Real Roots of a Trigonometric-Polynomial/fig/root_function_fig.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{fig/root_funtion_fig.pdf}
    \caption{The figure of the terminal-root-functions of $g$. 
    The red dotted line shows the graph of the start-point $x=M$ and the graphs of the terminal-root-functions are plotted as blue curves.
    }
    \label{fig:graph-Terminal-Root-Function}
\end{figure}


==> Isolating all the Real Roots of a Trigonometric-Polynomial/table/chen.tex <==
\begin{table}[ht]
\scriptsize
    \centering
    \scalebox{0.55}{
    \begin{tabular}{|c|c|c|c|c|c|c|c||c|c|c|c|c|c|c|c|}
\hline
Example&$k_{-}$&$k_{+}$&PRoots&BRoots&wSeq&wTime&Time&Example&$k_{-}$&$k_{+}$&PRoots&BRoots&wSeq&wTime&Time\\
\hline
\cite[Ex.1]{chen2022automated}&-1&1&4(1)&7(1)&6;5;5;6&0.005s&0.251s&
\cite[Ex.2]{chen2022automated}&0&0&-&1(5)&6;5;5;6&0.006s&0.054s\\
\hline
\cite[Ex.4]{chen2022automated}&0&0&1(2)&-&-&0s&0.003s&
\cite[Ex.1, $k=1$]{chenliu2016} &0&0&4(1)&1(3)&8;7;7;8&0.009s&0.075s\\
\hline
\cite[Ex.1, $k=2$]{chenliu2016}&0&0&4(1)&1(5)&8;7;7;8&0.009s&0.058s&
\cite[Ex.1, $k=3$]{chenliu2016}&0&0&4(1)&1(3);2(1)&8;7;7;8&0.01s&0.085s\\
\hline
\cite[Ex.2, $c=9/45$]{chenliu2016}&-1&1&4(1)&1(6);6(1)&21;43;43;21&0.124s&1.089s&
\cite[Ex.2, $c=8/45$]{chenliu2016}&-1&1&4(1)&1(8);6(1)&21;43;43;21&0.084s&1.065s\\
\hline
\cite[Ex.2, $c=7/45$]{chenliu2016}&-1&1&4(1)&1(6);4(1)&21;43;43;21&0.123s&1.013s&
\cite[Ex.2, $c=6/45$]{chenliu2016}&-1&1&4(1)&1(6);4(1)&21;43;43;21&0.074s&0.964s\\
\hline
\cite[Ex.3]{chenliu2016}&-3&3&4(1)&1(5);12(1)&28;51;51;28&0.238s&1.719s&
\cite[Ex.4]{chenliu2016}&0&0&4(1)&1(8)&6;6;6;6&0.005s&0.246s\\
\hline
\cite[Ex.5]{chenliu2016}&0&0&-&2(1)&7;7;7;7&0.007s&0.098s&
\cite[Ex.6]{chenliu2016}&0&0&4(1)&1(7)&17;15;15;17&0.053s&0.18s\\
\hline
\cite[Ex.7]{chenliu2016}&0&0&-&1(5)&6;5;5;6&0.005s&0.048s&
\cite[Ex.8]{chenliu2016}&-1&1&4(1)&1(2);4(1)&4;3;3;4&0.001s&0.129s\\
\hline
\cite[Ex.9]{chenliu2016}&0&1&-&1(2)&5;5;5;5&0.005s&0.138s&
\cite[Ex.10]{chenliu2016}&0&0&4(1)&1(3)&8;7;7;8&0.056s&0.105s\\
\hline
\cite[Ex.11]{chenliu2016}&0&0&-&1(1)&4;4;4;4&0.003s&0.042s&
\cite[Ex.12]{chenliu2016}&-1&1&4(1)&8(1)&7;8;8;7&0.006s&0.187s\\
\hline
\cite[Ex.13]{chenliu2016}&0&0&4(1)&1(3)&8;7;7;8&0.007s&0.053s&&&&&&&&\\
\hline

% \hline
% Example & $k_{-}$ & $k_{+}$ & PRoots & BRoots    &Time 
% & Example & $k_{-}$ & $k_{+}$ & PRoots & BRoots    &Time\\
% \hline
% \cite[Ex.1]{chen2022automated}    &0  &0  &4(1)    &3(1)      &0.28s&\cite[Ex.2]{chen2022automated}     &0  &0  &-       &1(5)      &0.25s\\
% \hline
% \cite[Ex.4]{chen2022automated}     &0  &0  &1(2)    &-         &0.14s
% &\cite[Ex.1, $k=1$]{chenliu2016}     &0  &0  &4(1)    &1(3)      &0.38s\\
% \hline
% \cite[Ex.1, $k=2$]{chenliu2016}     &0  &0  &4(1)    &1(5)      &0.31s
% &\cite[Ex.1, $k=3$]{chenliu2016}    &0  &0  &4(1)    &1(3);2(1) &0.33s\\
% \hline
% \cite[Ex.2, $c=9/45$]{chenliu2016}     &-1 &1  &4(1)    &1(6);6(1) &1.98s
% &\cite[Ex.2, $c=8/45$]{chenliu2016}      &-1 &1  &4(1)    &1(8);6(1) &1.84s\\
% \hline
% \cite[Ex.2, $c=7/45$]{chenliu2016}      &-1 &1  &4(1)    &1(6);4(1) &1.84s
% &\cite[Ex.2, $c=6/45$]{chenliu2016}    &-1 &1  &4(1)    &1(6);4(1) &2.96s\\
% \hline
% \cite[Ex.3]{chenliu2016}     &0  &0  &4(1)    &1(5)      &1.26s
% &\cite[Ex.4]{chenliu2016}     &0  &0  &4(1)    &1(4)      &0.73s\\
% \hline
% \cite[Ex.5]{chenliu2016}     &0  &0  &-       &2(1)      &0.38s
% &\cite[Ex.6]{chenliu2016}     &0  &0  &4(1)    &1(7)      &0.41s\\
% \hline
% \cite[Ex.7]{chenliu2016}     &0  &0  &-       &1(5)      &0.31s
% &\cite[Ex.8]{chenliu2016}     &0  &0  &4(1)    &1(2);2(1) &0.30s\\
% \hline
% \cite[Ex.9]{chenliu2016}     &0  &1  &-       &1(2)      &0.33s
% &\cite[Ex.10]{chenliu2016}     &0  &0  &4(1)    &1(3)      &0.27s\\
% \hline
% \cite[Ex.11]{chenliu2016}    &0  &0  &-       &1(1)      &0.29s
% &\cite[Ex.12]{chenliu2016}     &-1 &1  &4(1)    &8(1)      &0.31s\\
% \hline
% \cite[Ex.13]{chenliu2016}     &0  &0  &4(1)    &1(3)      &0.28s&     &   &  &        &         &\\
% \hline
    \end{tabular}}
    \caption{Results for Examples from the Literature (s: seconds).}
    \label{tab:chen-result}
\end{table}

==> Isolating all the Real Roots of a Trigonometric-Polynomial/table/notation.tex <==
\begin{table}[ht]
\scriptsize
    \centering
    \scalebox{0.75}{
    \begin{tabular}{|c|c|}
\hline
$k_{-}$ & an integer such that $2k_{-}\pi-\pi$ is a lower bound for all bounded real roots\\
\hline
$k_{+}$ & an integer such that $2k_{+}\pi+\pi$ is an upper bound for all bounded real roots
\\
\hline
PRoots & periodic real roots\\
\hline
BRoots & bounded real roots\\
\hline
wSeq & the lengths of four computed weak Fourier sequences \\
\hline
wTime & time for computing four weak Fourier sequences\\
\hline
Time & total computing time \\
\hline
$n(m)$ & the number of bunches of periodic real roots / 
the number of bounded real roots (the multiplicity of each root)\\
% the example has $n_i$ periodic (bounded) real roots and the multiplicity of each is $m_i$ for $i=1,\ldots,t$\\
% $n_1(m_1);\ldots;n_t(m_t)$ & the example has $n_i$ periodic (bounded) real roots and the multiplicity of each is $m_i$ for $i=1,\ldots,t$\\
\hline
-&no periodic or bounded real roots / no need to compute weak Fourier sequences\\
\hline
% OT&out of the timing 3600 seconds\\
% \hline
    \end{tabular}}
    \caption{Notation.} %\textcolor{red}{(Tianqi: There are at least $k$ roots in the interval $(2k_{-}\pi-\pi,2k_{+}\pi+\pi)$)}
    \label{tab:notation}
\end{table}

==> Isolating all the Real Roots of a Trigonometric-Polynomial/table/random.tex <==
\begin{table}[ht]
\scriptsize
    \centering
    \scalebox{0.45}{
    \begin{tabular}{|c|c|c|c|c|c|c|c||c|c|c|c|c|c|c|c|}
\hline
Example&$k_{-}$&$k_{+}$&PRoots&BRoots&wSeq&wTime&Time&Example&$k_{-}$&$k_{+}$&PRoots&BRoots&wSeq&wTime&Time\\
\hline
$M_{1}$&0&0&-&2(1)&27;27;27;27&0.186s&0.532s&$M_{2}$&0&0&4(1)&4(1)&26;26;26;26&0.148s&0.634s\\
\hline
$M_{3}$&0&0&4(1)&2(1)&22;24;24;22&0.08s&0.286s&$M_{4}$&-3&3&4(1)&15(1)&18;14;14;18&0.032s&0.592s\\
\hline
$M_{5}$&0&2&8(1)&11(1)&16;20;20;16&0.054s&0.542s&$M_{6}$&0&0&4(1)&4(1)&29;53;53;29&0.212s&0.62s\\
\hline
$M_{7}$&0&0&7(1)&2(1)&20;20;20;20&0.078s&0.361s&$M_{8}$&-2&2&4(1)&11(1)&49;26;26;49&0.215s&1.402s\\
\hline
$M_{9}$&-1&1&6(1)&7(1)&39;21;21;39&0.146s&0.878s&$M_{10}$&0&0&-&-&13;12;12;13&0.013s&0.101s\\
\hline
$M_{11}$&0&0&10(1)&5(1)&99;88;88;99&1.325s&2.167s&$M_{12}$&0&0&5(1);2(2)&1(1)&-&0s&0.018s\\
\hline
$M_{13}$&0&0&3(1)&4(1)&53;54;54;53&0.421s&1.367s&$M_{14}$&0&0&2(1)&1(4)&-&0s&0.009s\\
\hline
$M_{15}$&-1&1&4(1)&9(1)&87;192;192;87&2.765s&8.305s&$M_{16}$&-1&0&12(1)&15(1)&175;174;174;175&4.416s&13.173s\\
\hline
$M_{17}$&0&0&2(2)&1(2)&-&0s&0.001s&$M_{18}$&0&0&3(2)&1(3);1(1)&20;23;23;20&0.06s&0.238s\\
\hline
$M_{19}$&-5&1&10(1)&29(1)&70;212;212;70&3.87s&15.224s&$M_{20}$&0&0&3(8)&1(10)&-&0s&0.001s\\
\hline
$M_{21}$&0&1&-&2(1)&107;107;107;107&1.566s&7.036s&$M_{22}$&0&0&-&1(2);2(1)&79;79;79;79&1.001s&3.233s\\
\hline
$M_{23}$&-1&1&12(1)&16(1)&216;195;195;216&5.432s&23.089s&$M_{24}$&-4&4&4(1)&20(1)&104;213;213;104&4.035s&22.34s\\
\hline
$M_{25}$&0&0&8(1)&4(1)&107;243;243;107&5.278s&9.108s&$M_{26}$&-1&2&8(1)&16(1)&193;154;154;193&5.656s&19.36s\\
\hline
$M_{27}$&-2&2&8(1)&26(1)&143;161;161;143&4.508s&19.111s&$M_{28}$&0&0&-&1(2);1(1)&92;92;92;92&1.49s&2.893s\\
\hline
$M_{29}$&-1&1&8(1)&12(1)&108;177;177;108&3.516s&10.417s&$M_{30}$&0&1&4(1)&5(1)&99;233;233;99&4.659s&10.586s\\
\hline
$M_{31}$&0&0&4(1)&2(1)&103;247;247;103&5.227s&7.974s&$M_{32}$&0&1&4(1)&6(1)&105;249;249;105&5.022s&14.39s\\
\hline
$M_{33}$&-1&1&8(1)&12(1)&250;97;97;250&7.234s&19.997s&$M_{34}$&0&0&4(1)&4(1)&270;111;111;270&6.47s&11.022s\\
\hline
$M_{35}$&-1&1&8(1)&12(1)&535;111;111;535&55.14s&83.45s&$M_{36}$&0&0&4(1)&1(1)&259;106;106;259&8.499s&10.169s\\
\hline
$M_{37}$&0&1&4(1)&3(1)&103;260;260;103&7.776s&11.775s&$M_{38}$&0&0&4(1)&5(1)&100;100;100;100&1.575s&4.608s\\
\hline
$M_{39}$&0&1&4(1)&4(1)&103;103;103;103&2.115s&6.234s&$M_{40}$&-1&1&4(1)&7(1)&232;104;104;232&4.875s&12.368s\\
\hline
$M_{41}$&0&0&-&1(1)&74;90;90;74&1.325s&1.669s&$M_{42}$&-1&1&4(1)&1(5);10(1)&521;204;204;521&43.424s&84.569s\\
\hline
$M_{43}$&0&0&4(1)&1(6);3(1)&106;51;51;106&0.787s&1.46s&$M_{44}$&-6&6&8(1)&1(6);53(1)&463;382;382;463&44.619s&374.288s\\
\hline
$M_{45}$&0&0&4(1)&1(3);2(1)&183;611;611;183&97.672s&116.082s&$M_{46}$&-1&1&8(1)&1(2);13(1)&283;95;95;283&10.331s&29.126s\\
\hline
$M_{47}$&0&0&8(1)&2(1)&167;218;218;167&13.509s&17.624s&$M_{48}$&-1&1&10(1)&13(1)&336;538;538;336&70.131s&190.27s\\
\hline
$M_{49}$&0&0&2(1)&1(3)&84;91;91;84&1.13s&2.598s&$M_{50}$&-1&2&11(1)&17(1)&141;151;151;141&5.713s&19.468s\\
\hline
$M_{51}$&-2&1&8(1)&14(1)&200;905;905;200&230.777s&610.059s&$M_{52}$&0&0&-&1(2);2(1)&223;223;223;223&7.84s&19.67s\\
\hline
$M_{53}$&0&0&4(1)&1(2);5(1)&709;222;222;709&140.087s&173.988s&$M_{54}$&-1&1&8(1)&10(1)&605;787;787;605&233.809s&518.236s\\
\hline
$M_{55}$&0&1&-&2(1)&197;197;197;197&7.109s&25.48s&$M_{56}$&0&0&4(1)&1(4)&219;219;219;219&6.292s&16.779s\\
\hline
$M_{57}$&0&0&-&4(1)&223;223;223;223&7.016s&25.085s&$M_{58}$&-1&1&8(1)&1(2);14(1)&701;593;593;701&126.757s&368.925s\\
\hline
$M_{59}$&0&0&-&1(2);3(1)&230;230;230;230&10.187s&24.844s&$M_{60}$&-1&1&8(1)&12(1)&1133;219;219;1133&382.221s&806.921s\\
\hline
$M_{61}$&-1&0&4(1)&7(1)&245;650;650;245&60.368s&153.185s&$M_{62}$&0&0&-&4(1)&233;233;233;233&11.5s&32.585s\\
\hline
$M_{63}$&-1&1&4(1)&8(1)&243;617;617;243&50.81s&146.751s&$M_{64}$&-1&1&4(1)&7(1)&565;236;236;565&44.672s&97.59s\\
\hline
$M_{65}$&-7&7&4(1)&31(1)&234;537;537;234&43.514s&284.004s&$M_{66}$&0&1&4(1)&1(2);8(1)&237;597;597;237&52.063s&121.855s\\
\hline
$M_{67}$&-1&1&8(1)&13(1)&236;616;616;236&53.379s&171.749s&$M_{68}$&-1&1&4(1)&10(1)&242;631;631;242&50.009s&162.565s\\
\hline
$M_{69}$&-1&0&4(1)&5(1)&612;234;234;612&58.078s&91.915s&$M_{70}$&-1&0&4(1)&5(1)&609;238;238;609&52.149s&102.304s\\
\hline
$M_{71}$&0&0&3(1)&1(8);2(1)&164;164;164;164&3.571s&6.428s&$M_{72}$&-1&0&3(6);2(2);4(1)&1(13);6(1)&30;32;32;30&0.13s&5.488s\\
\hline
$M_{73}$&0&0&3(4);2(1)&1(6);3(1)&122;122;122;122&2.128s&4.072s&$M_{74}$&0&0&3(5);4(1)&1(7);5(1)&120;309;309;120&11.067s&23.141s\\
\hline
$M_{75}$&0&0&3(4)&1(4)&86;96;96;86&1.869s&2.906s&$M_{76}$&-1&0&15(1)&9(1)&1005;385;385;1005&338.574s&940.537s\\
\hline
$M_{77}$&-1&0&3(2);2(3);4(1)&1(4);2(1)&34;42;42;34&0.274s&0.819s&$M_{78}$&0&0&3(3);4(1)&1(7);3(1)&168;437;437;168&36.463s&45.945s\\
\hline
$M_{79}$&0&0&7(1)&1(2);1(1)&278;803;803;278&161.677s&170.291s&$M_{80}$&0&0&13(1)&1(4)&767;1009;1009;767&515.406s&518.845s\\
\hline
$M_{81}$&-1&0&-&4(1)&23;20;20;23&0.07s&0.379s&$M_{82}$&0&0&4(1)&2(1)&31;22;22;31&0.095s&0.298s\\
\hline
$M_{83}$&0&0&8(1)&3(1)&50;53;53;50&0.35s&0.787s&$M_{84}$&0&0&-&1(2);3(1)&17;18;18;17&0.104s&0.532s\\
\hline
$M_{85}$&0&0&4(1)&1(2);2(1)&16;14;14;16&0.04s&0.15s&$M_{86}$&0&0&-&3(1)&28;28;28;28&0.185s&0.739s\\
\hline
$M_{87}$&-1&1&11(1)&14(1)&17;18;18;17&0.049s&0.61s&$M_{88}$&0&0&-&1(2);1(1)&30;30;30;30&0.188s&0.588s\\
\hline
$M_{89}$&0&0&-&1(1)&19;19;19;19&0.109s&0.355s&$M_{90}$&-1&1&4(1)&6(1)&28;51;51;28&0.241s&1.035s\\
\hline
$M_{91}$&-1&0&-&1(2);1(1)&58;49;49;58&0.69s&2.015s&$M_{92}$&0&0&3(1)&1(7)&55;55;55;55&0.533s&1.269s\\
\hline
$M_{93}$&0&0&5(2);4(1)&1(3);2(1)&20;17;17;20&0.062s&0.243s&$M_{94}$&0&0&5(2)&1(6)&-&0s&0.002s\\
\hline
$M_{95}$&0&0&3(5)&1(9)&-&0s&0.0s&$M_{96}$&0&0&6(1)&1(6);1(1)&155;67;67;155&1.855s&2.914s\\
\hline
$M_{97}$&0&0&3(2);2(3)&1(5)&-&0s&0.006s&$M_{98}$&0&0&13(1)&5(1)&46;38;38;46&0.24s&0.667s\\
\hline
$M_{99}$&-10&10&6(1)&1(3);24(1)&5;5;5;5&0.003s&0.818s&$M_{100}$&0&0&4(1)&1(4);4(1)&28;48;48;28&0.205s&0.627s\\
\hline
$M_{101}$&0&0&-&1(2)&88;88;88;88&1.345s&3.151s&$M_{102}$&0&13&4(1)&1(3);78(1)&320;88;88;320&11.792s&95.276s\\
\hline
$M_{103}$&-7&7&8(1)&1(2);58(1)&327;87;87;327&15.814s&98.576s&$M_{104}$&-3&2&12(1)&32(1)&202;307;307;202&11.731s&66.217s\\
\hline
$M_{105}$&-1&0&7(1)&1(3);3(1)&94;222;222;94&4.1s&8.278s&$M_{106}$&-1&1&8(1)&9(1)&223;98;98;223&8.054s&16.822s\\
\hline
$M_{107}$&-1&0&8(1)&6(1)&335;242;242;335&14.961s&29.263s&$M_{108}$&0&0&8(1)&5(1)&179;175;175;179&8.592s&11.608s\\
\hline
$M_{109}$&-2&2&8(1)&21(1)&237;100;100;237&4.992s&28.19s&$M_{110}$&-1&0&-&1(1)&68;68;68;68&0.871s&3.634s\\
\hline
$M_{111}$&-1&1&4(1)&7(1)&110;245;245;110&5.441s&20.069s&$M_{112}$&-1&0&-&3(1)&82;82;82;82&1.066s&2.765s\\
\hline
$M_{113}$&-1&1&8(1)&13(1)&266;286;286;266&12.064s&42.789s&$M_{114}$&-1&0&4(1)&5(1)&107;245;245;107&6.711s&12.651s\\
\hline
$M_{115}$&-1&1&4(1)&7(1)&104;253;253;104&5.52s&15.223s&$M_{116}$&-1&4&8(1)&24(1)&271;271;271;271&14.857s&66.69s\\
\hline
$M_{117}$&-1&0&-&1(1)&104;104;104;104&1.941s&5.852s&$M_{118}$&-1&1&8(1)&8(1)&431;111;111;431&32.513s&49.383s\\
\hline
$M_{119}$&-1&0&4(1)&6(1)&111;279;279;111&11.232s&19.781s&$M_{120}$&0&0&-&-&107;107;107;107&1.763s&3.846s\\
\hline
$M_{121}$&-1&1&4(1)&8(1)&397;151;151;397&13.506s&39.123s&$M_{122}$&0&0&11(1)&1(10);4(1)&1443;182;182;1443&1273.551s&1766.71s\\
\hline
$M_{123}$&-6&0&17(1)&1(3);30(1)&833;543;543;833&267.967s&1832.919s&$M_{124}$&-68&1&6(1)&1(3);141(1)&151;623;623;151&88.491s&1008.551s\\
\hline
$M_{125}$&0&0&10(1)&3(1)&429;389;389;429&43.514s&65.364s&$M_{126}$&0&1&8(1)&6(1)&499;981;981;499&292.23s&870.745s\\
\hline
$M_{127}$&-1&1&2(2);4(1)&1(2);8(1)&311;129;129;311&25.591s&35.585s&$M_{128}$&0&0&-&3(1)&32;32;32;32&0.396s&0.928s\\
\hline
$M_{129}$&-1&1&8(1)&11(1)&132;132;132;132&2.595s&12.191s&$M_{130}$&-1&0&10(1)&1(3);10(1)&329;448;448;329&48.12s&93.598s\\
\hline
$M_{131}$&0&0&8(1)&5(1)&687;661;661;687&153.159s&249.382s&$M_{132}$&-1&0&4(1)&5(1)&225;560;560;225&40.575s&79.235s\\
\hline
$M_{133}$&0&0&-&4(1)&217;217;217;217&12.072s&23.128s&$M_{134}$&-1&1&8(1)&10(1)&513;1395;1395;513&1017.194s&2496.384s\\
\hline
$M_{135}$&-1&1&4(1)&6(1)&547;225;225;547&40.101s&99.09s&$M_{136}$&-1&1&8(1)&12(1)&649;533;533;649&106.612s&259.645s\\
\hline
$M_{137}$&0&1&4(1)&6(1)&623;241;241;623&58.741s&98.687s&$M_{138}$&-3&3&8(1)&1(2);28(1)&503;459;459;503&72.135s&325.427s\\
\hline
$M_{139}$&0&0&4(1)&4(1)&595;607;607;595&105.192s&138.137s&$M_{140}$&0&0&-&2(1)&215;215;215;215&8.132s&26.755s\\
\hline
$M_{141}$&0&0&4(1)&4(1)&242;621;621;242&60.554s&102.052s&$M_{142}$&-23&1&8(1)&18(1)&240;1361;1361;240&574.013s&1821.513s\\
\hline
$M_{143}$&-1&0&4(1)&6(1)&245;245;245;245&10.063s&55.621s&$M_{144}$&-1&1&4(1)&9(1)&227;586;586;227&51.978s&140.508s\\
\hline
$M_{145}$&0&0&-&1(1)&246;246;246;246&10.292s&32.055s&$M_{146}$&0&1&8(1)&8(1)&226;607;607;226&67.49s&115.328s\\
\hline
$M_{147}$&-4&4&4(1)&18(1)&247;647;647;247&55.513s&278.322s&$M_{148}$&-1&0&4(1)&4(1)&245;645;645;245&69.837s&131.675s\\
\hline
$M_{149}$&-1&0&8(1)&7(1)&234;630;630;234&73.299s&138.112s&$M_{150}$&0&1&12(1)&9(1)&1117;610;610;1117&542.28s&1267.414s\\
\hline
$M_{151}$&0&0&3(6);6(1)&1(13);2(1)&46;46;46;46&0.604s&1.933s&$M_{152}$&0&0&11(1)&1(4);2(1)&154;856;856;154&455.72s&663.41s\\
\hline
$M_{153}$&0&0&4(1)&1(3);1(1)&170;430;430;170&27.564s&43.251s&$M_{154}$&0&0&3(10);2(5)&1(12)&-&0s&0.023s\\
\hline
$M_{155}$&0&0&3(5);4(1)&1(5);2(1)&25;35;35;25&0.163s&0.568s&$M_{156}$&0&0&2(2);8(1)&4(1)&200;635;635;200&235.405s&275.278s\\
\hline
$M_{157}$&-1&1&4(1)&6(1)&433;213;213;433&15.891s&26.104s&$M_{158}$&0&0&2(3);4(1)&5(1)&94;138;138;94&3.508s&9.013s\\
\hline
$M_{159}$&-1&15&6(1)&64(1)&345;145;145;345&12.958s&168.032s&$M_{160}$&-1&1&11(1);2(2)&1(3);10(1)&203;279;279;203&15.479s&30.66s\\
\hline

    \end{tabular}}
    \caption{Results for Random Examples (s: seconds).}
    \label{tab:random-result}
\end{table}
